Parallel Successive Learning for Dynamic Distributed Model Training over Heterogeneous Wireless Networks

Federated learning (FedL) has emerged as a popular technique for distributing model training over a set of wireless devices, via iterative local updates (at devices) and global aggregations (at the server). In this paper, we develop parallel successive learning (PSL), which expands the FedL architecture along three dimensions: (i) Network, allowing decentralized cooperation among the devices via device-to-device (D2D) communications. (ii) Heterogeneity, interpreted at three levels: (ii-a) Learning: PSL considers heterogeneous number of stochastic gradient descent iterations with different mini-batch sizes at the devices; (ii-b) Data: PSL presumes a dynamic environment with data arrival and departure, where the distributions of local datasets evolve over time, captured via a new metric for model/concept drift. (ii-c) Device: PSL considers devices with different computation and communication capabilities. (iii) Proximity, where devices have different distances to each other and the access point. PSL considers the realistic scenario where global aggregations are conducted with idle times in-between them for resource efficiency improvements, and incorporates data dispersion and model dispersion with local model condensation into FedL. Our analysis sheds light on the notion of cold vs. warmed up models, and model inertia in distributed machine learning. We then propose network-aware dynamic model tracking to optimize the model learning vs. resource efficiency tradeoff, which we show is an NP-hard signomial programming problem. We finally solve this problem through proposing a general optimization solver. Our numerical results reveal new findings on the interdependencies between the idle times in-between the global aggregations, model/concept drift, and D2D cooperation configuration.

==> ProofThLoss.tex <==
(currently I am assuming the nodes have the same number of datapoints for simplicity)
%  We start the proof by recursively expanding the local updates, which results in the following expression for the weight obtained at the last local update:
% \begin{equation}
%     \mathbf{w}^{(k-1)}_{i,E_i}= \mathbf{w}^{(k-1)}- \frac{\eta_i}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}
% Consequently, the global aggregation given in~\eqref{eq:globAgg} can be written as:
% \begin{equation}
%     \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta_i}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}
% The above update can be expressed in terms of a centralized gradient descent update with an additional noise term as follows:
% \begin{equation}\label{eq:update1}
%     \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta_i}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) + e^{(k)} = \mathbf{w}^{(k-1)}-\eta_i\nabla F_i(\mathbf{w}^{(k-1)}) + e^{(k)},
% \end{equation}
% where the error term is given by:
% \begin{equation}
%     e^{(k)}=\frac{\eta_i}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta_i}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}


% Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
% \begin{equation}\label{eq:quadBound}
%  \begin{aligned}
%      F_i(\mathbf{w}^{(k)})\leq& F_i(\mathbf{w}^{(k-1)})+ (\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)})^\top \nabla F_i(\mathbf{w}^{(k-1)})+\frac{L}{2}\norm{\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)}}^2.
%      \end{aligned}
%  \end{equation}
%  By replacing the update rule given in~\eqref{eq:update1} in the above inequality, we get:
%  \begin{equation}
%       \begin{aligned}
%      F_i(\mathbf{w}^{(k)})\leq& F_i(\mathbf{w}^{(k-1)})+ (-\eta_i\nabla F_i(\mathbf{w}^{(k-1)}) + e^{(k)})^\top \nabla F_i(\mathbf{w}^{(k-1)})
%      +\frac{L}{2}\norm{-\eta_i\nabla F_i(\mathbf{w}^{(k-1)}) + e^{(k)}}^2.
%      \end{aligned}
%  \end{equation}
%  Performing some algebraic manipulations on the above inequality yields:
%   \begin{equation}
%       \begin{aligned}
%      F_i(\mathbf{w}^{(k)})\leq& F_i(\mathbf{w}^{(k-1)})- \eta_i \Vert\nabla F_i(\mathbf{w}^{(k-1)})\Vert^2 + e^{(k)^\top} \nabla F_i(\mathbf{w}^{(k-1)})\\&
%      +\frac{L}{2}\left(\eta_i^2\Vert\nabla F_i(\mathbf{w}^{(k-1)})\Vert^2+\Vert e^{(k)}\Vert^2-2\eta_i e^{(k)^\top}\nabla F_i(\mathbf{w}^{(k-1)})\right).
%      \end{aligned}
%  \end{equation}
%  Thus, we have:
%  \begin{equation}
%      \begin{aligned}
%          F_i(\mathbf{w}^{(k)})\leq& F_i(\mathbf{w}^{(k-1)})+ \left(\frac{L\eta_i^2}{2} -\eta_i\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)})\Vert^2 + \left(1-L\eta_i \right)e^{(k)^\top} \nabla F_i(\mathbf{w}^{(k-1)})
%      +\frac{L}{2}\Vert e^{(k)}\Vert^2.
%      \end{aligned}
%  \end{equation}
%  For a given weight spread at the beginning of the $k$-th global aggregation among the devices, i.e., $\mathbf{w}^{(k-1)}$, we take the expectation from the both hand sides of the above inequality, which yields:
%  \begin{equation}\label{eq:49}
%  \hspace{-5mm}
%      \begin{aligned}
%          \mathbb{E}_{k-1} [F_i(\mathbf{w}^{(k)})]\leq& F_i(\mathbf{w}^{(k-1)})+ \underbrace{ \left(\frac{L\eta_i^2}{2} -\eta_i\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)})\Vert^2}_{(a)} + \underbrace{\left(1-L\eta_i \right)\mathbb{E}_{k-1}[e^{(k)^\top}] \nabla F_i(\mathbf{w}^{(k-1)})}_{(b)}
%      +\underbrace{\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]}_{(c)}.
%      \end{aligned}
%      \hspace{-5mm}
%  \end{equation}
%  It can be seen that the above bound gives us the one step decrease of the value of the global loss function, which is what we desire. To further characterize the bound, we  carefully investigate terms (a), (b), and (c) appearing on the right hand side of the above inequality. 
 
%  \textbf{Term (a) in~\eqref{eq:49}}: Starting from term (a), noting that the algorithm should work when $\eta_i$ is sufficiently small, the coefficient of the norm square of gradient is negative for sufficiently small step sizes. To avoid sign change in the coefficient, we 
%  tune the step size such that $\frac{L\eta_i^2}{2} -\eta_i <0$, implying $\eta_i \leq 2/L$. As a result, to obtain an upper bound for (a), we need to find a lower bound on the norm square of the gradient. Using the strong convexity property, we have:
%  \begin{equation}
%         \norm{\nabla F_i(\mathbf{w}^{(k-1)})}^2 \geq \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star})\right){2\mu}.
%  \end{equation}
%  Thus, we get:
%  \begin{equation}
%      (a) \leq \mu \left({ L\eta_i^2} -2\eta_i\right)\left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star})\right).
%  \end{equation}
 
%  {\color{blue} We wanna maximize this term: Initial approach: \textbf{Term (b) in~\eqref{eq:49}}: For term (b), noting that the selection of the data points for each batch of SGD is conducted uniformly at random without replacement, SGD is an unbiased estimate of the true gradient. This implies the following equality:
%  \begin{equation}
%  \begin{aligned}
%      & \mathbb E_{k-1}[ e^{(k)}]=\frac{\eta_i}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\mathbb E_{t-1}\left[\frac{\eta_i}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\right]\\
%       &=\frac{\eta_i}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta_i}{N}\sum_{i=1}^{N} \frac{1}{E_iD_i}\sum_{e=1}^{E_i}\sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\\
%       &=\eta_i \nabla F_i(\mathbf{w}^{(k-1)})- \frac{\eta_i}{E_i}\sum_{e=1}^{E_i}\nabla  F_i(\mathbf{w}^{(k-1)}_{i,e-1}),
%       \end{aligned}
%       \hspace{-15mm}
%  \end{equation}
%  based on which we get:
%  \begin{equation}\label{eq:60s}
%  \begin{aligned}
%     &(b)=  \eta_i\left(1-L\eta_i \right) \Vert \nabla F_i(\mathbf{w}^{(k-1)})\Vert^2 -\eta_i\left(1-L\eta_i \right)\frac{\sum_{e=1}^{E_i} < \nabla  F_i(\mathbf{w}^{(k-1)}_{i,e-1}), \nabla F_i(\mathbf{w}^{(k-1)})>}{E_i}.
%     \end{aligned}
%  \end{equation}
%  Since the method should work with sufficiently small values of step size, to avoid sign changes we impose $\eta_i\leq 1/L$, which implies $1-L\eta_i \geq 0$. Noting that for any two vectors $a$, $b$, we have $-<a,b> ~\leq ||a||\times  ||b||$, \eqref{eq:60s} can be written as:
%   \begin{equation}\label{eq:60s}
%  \begin{aligned}
%     &(b)\leq \eta_i\left(1-L\eta_i \right) \Vert \nabla F_i(\mathbf{w}^{(k-1)})\Vert^2\\& +\eta_i\left(1-L\eta_i \right)\frac{\sum_{e=1}^{E_i} \Vert \nabla  F_i(\mathbf{w}^{(k-1)}_{i,e-1})\Vert \times \Vert \nabla F_i(\mathbf{w}^{(k-1)})\Vert}{E_i}\\&
%     \leq \eta_i\left(1-L\eta_i \right) L^2 \Vert \mathbf{w}^{(k-1)} - \mathbf{w}^{{(k-1)}^\star}\Vert^2\\& +\eta_i\left(1-L\eta_i \right)\frac{L^2\sum_{e=1}^{E_i} \Vert   \mathbf{w}^{(k-1)}_{i,e-1} -\mathbf{w}^{{(k-1)}^\star} \Vert \times \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{{(k-1)}^\star} \Vert}{E_i}
%     \end{aligned}
%  \end{equation}
%  We leave this expression here and get back to it later in the proof. (TO DO!)}
 
%  \textbf{Term (c) in~\eqref{eq:49}}: This term is given by:
%  \begin{equation}\label{52}
%      \begin{aligned}
%     & (c)=\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]=\frac{L}{2}\mathbb{E}_{k-1} \Big\Vert\frac{\eta_i}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta_i}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\ 
%      &
%      =\frac{L}{2} \frac{\eta_i^2}{N^2} \mathbb{E}_{k-1}\Big\Vert\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 
%      \\&
%      \leq \frac{L}{2} \frac{\eta_i^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 .
%      \end{aligned}
%  \end{equation}
%  The last inequality is a result of Cauchy–Schwarz inequality, desribed by $<\textbf{a},\textbf{a}'>~\leq \norm{\textbf{a}}.\norm{\textbf{a}'}$, which results in the following bound, where $\mathbf{q}=[q_1,\cdots,q_b]$:
% \begin{equation}
% \begin{aligned}
%     &\left(\sum_{a=1}^{b} q_i \right)^2= \left(<\mathbf{1},\mathbf{q}> \right)^2
%     \leq b \sum_{a=1}^{b} q^2_i.
%     \end{aligned}
% \end{equation} 
% The next step is to further bound~\eqref{52}. We take the following steps:
% \begin{equation}\label{eq:54}
%     \begin{aligned}
%         &\frac{L}{2} \frac{\eta_i^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\
%         &\overset{(i)}{=}\frac{L}{2} \frac{\eta_i^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Bigg\Vert\left(\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\right)\\
%         &- \left(\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \right) \Bigg\Vert^2\\
%         &\overset{(ii)}{\leq} \frac{{L}\eta_i^2}{N}\sum_{i=1}^{N} \underbrace{\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d)} \\
%         &+\frac{{L}\eta_i^2}{N}\sum_{i=1}^{N}\underbrace{\mathbb{E}_{k-1} \Bigg\Vert\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})  \Bigg\Vert^2}_{(e)},
%     \end{aligned}
%     \hspace{-10mm}
% \end{equation}
% where in (i) we have added and subtracted the same term inside the norm and (ii) is the result of Cauchy–Schwarz inequality  described above. Now, we focus on each of these terms and try to further bound them:
% \begin{equation}\label{eq:55}
%     \begin{aligned}
%         (d) &=\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         =\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{E_i}\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         =\frac{1}{E^2_i}\mathbb{E}_{k-1}\Bigg\Vert\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         \leq \frac{1}{E_i}\mathbb{E}_{k-1}\sum_{e=1}^{E_i} \underbrace{\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d')},
%     \end{aligned}
% \end{equation}
% where the last inequality is the result of Cauchy–Schwarz inequality  described above. Now, the above equation, resembles a known result in sampling theory. In $(d')$, the first term inside the norm is the \textit{true average of a population} and the second term is the \textit{sampled average of a population}. Thus, the last result of~\eqref{eq:55} can be considered as average of $E_i$ trail of variance of uniform sampling without replacement.
% We can use the result described in Section 2.8 of the book (Sampling:
% Design and Analysis
% Second Edition, written by
% Sharon L. Lohr). Using that result, we get:

% \begin{equation}
%     (d')= \left(1-\frac{B_i}{D_i}\right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) - \nabla F_i (\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)} ,
% \end{equation}
%  and thus
% \begin{equation}
% \begin{aligned}
%     (d)&\leq \left( 1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)}.
%     \end{aligned}
% \end{equation}
% This result has two implications: (i) it shows that if the size of mini-batch $B_i$ is equal to the size of the local data set, i.e., $B_i=D_i$, the error vanishes, and (ii) it shows that the error is a function of internal heterogeneity of the local dataset. 

% Now, we turn into bounding the term (e). Term (e) corresponds to the error between (i) sequentially applying the SGD to the batches of data and where the SGD uses the result of the previous batch as the initial point for the next batch, and (ii) the case where the data is partitioned into different batches and the SGD is applied to all of the batches using the same initial points across the batches. We get:
%  \begin{equation}\label{eq:57}
%      \begin{aligned}
%      (e)&= \mathbb{E}_{k-1} \Bigg\Vert \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
%      = \frac{1}{\left(E_iB_i\right)^2}\mathbb{E}_{k-1}  \Bigg\Vert \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
%      \overset{(i)}{\leq}\frac{1}{E_iB_i} \mathbb{E}_{k-1} \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \Big\Vert  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Big\Vert^2\\&
%       \overset{(ii)}{\leq} \frac{L^2}{E_i} \mathbb{E}_{k-1}\sum_{e=1}^{E_i}  \Big\Vert  \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)} \Big\Vert^2,
%      \end{aligned}
%  \end{equation}
% where in (i) we used the Cauchy–Schwarz inequality as described previously, and (ii) is due to L-smoothness. The last term can be interpreted as conducting SGD on local dataset for $E_i$ epochs of minibatch size $B_i$ and then calculating the cumulative average squared error.

For each local function, for $e\geq 2$ we can write the update as:
\begin{equation}
\begin{aligned}
    \mathbf{w}^{(k-1)}_{i,e-1}&=  \mathbf{w}^{(k-1)}_{i,e-2} - \frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\\
    &= \mathbf{w}^{(k)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\underbrace{\left(\frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) \right)}_{\triangleq \epsilon_i},
    \end{aligned}
\end{equation}
In the above format, the local updates are written in terms of conducting a full batch GD with an added noise that is due to the minibatch SGD. Since the local functions are smooth, we have:
Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
\begin{equation}\label{eq:quadBound}
 \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ (\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2})^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})+\frac{L}{2}\norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2}}^2.
     \end{aligned}
 \end{equation}
 Consequently, we have:
 \begin{equation}
      \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ (-\eta_i\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i)^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\norm{-\eta_i\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i}^2.
     \end{aligned}
 \end{equation}
 Performing some algebraic manipulations on the above inequality yields:
  \begin{equation}
      \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})- \eta_i \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \epsilon_i^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\\&
     +\frac{L}{2}\left(\eta_i^2\Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2+\Vert \epsilon_i\Vert^2-2\eta_i \epsilon_i^\top\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right).
     \end{aligned}
 \end{equation}
 Thus, we get:
 \begin{equation}\label{eq:59}
     \begin{aligned}
         F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta_i^2}{2} -\eta_i\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \left(1-L\eta_i \right)\epsilon_i^{\top} \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
 \end{equation}
 Taking the expectation w.r.t the data sampling procedure at node $i$, since SGD is unbiased we have:
 \begin{equation}
     \mathbb{E} \left[ \frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right]=\frac{\eta_i}{D_i}  \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}),
 \end{equation}
implying:
\begin{equation}
    \mathbb{E}[ \epsilon_i]=0.
\end{equation}
Taking the expectation from both hand sides of~\eqref{eq:59} and applying the above result yields:
  \begin{equation}\label{eq:62}
       \hspace{-5mm}
     \begin{aligned}
        &\mathbb{E}_{e-2} [F_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta_i^2}{2} -\eta_i\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
     \hspace{-5mm}
 \end{equation}
  To avoid sign change in the second term of the right hand side, we 
 tune the step size such that $\frac{L\eta_i^2}{2} -\eta_i <0$, implying $\eta_i \leq 2/L$. Using the PL condition, we have:
 \begin{equation}
        \norm{\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2 \geq \left(F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right){2\mu},
 \end{equation}
 where $\mathbf{w}^{(k-1)^\star}_i$ denotes the local optimal point of the local dataset at node $i$.
 Replacing the above result in~\eqref{eq:62}, we get:
  \begin{equation}\label{eq:65}
     \begin{aligned}
        &\mathbb{E}_{e-2} [F_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \mu\left({L\eta_i^2} -2\eta_i\right)  (F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)) 
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i \Vert^2.
     \end{aligned}
 \end{equation}
Now we turn into calculating $\mathbb{E}_{e-2}[\Vert \epsilon_i \Vert^2]$ in the above expression. At each time instant, $\mathbb{E}_{e-2}[\Vert \epsilon_i\Vert^2]$ can be expressed as follows:
\begin{equation}\label{eq:66}
\begin{aligned}
    \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\mathbb{E}_{e-2}\Big\Vert\frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\eta_i^2\mathbb{E}_{e-2}\Big\Vert\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2.
    \end{aligned}
\end{equation}
To obtain the above expression, we use the result described in Section 2.8 of the book (Sampling:
Design and Analysis
Second Edition, written by
Sharon L. Lohr) and get:
\begin{equation}
\begin{aligned}
    \frac{1}{\eta_i^2} \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}
     \\
      &= \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{D_i}\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &= \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{1}{D^2_i} \left\Vert D_i\nabla  f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &\leq \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{(D_i-1)}{D_i} \Theta_i}{B_i(D_i-1)}=\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
\end{equation}
Replacing the above result in~\eqref{eq:65}, we get:
  \begin{equation}\label{eq:65_1}
     \begin{aligned}
        \mathbb{E}_{e-2} [F_i(\mathbf{w}^{(k-1)}_{i,e-1})]-F_i(\mathbf{w}^{(k-1)}_{i,e-2})&\leq \mu\left({L\eta_i^2} -2\eta_i\right) \left(F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right) 
     +\frac{L\eta_i^2}{2}\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
 \end{equation}
 Adding $F_i(\mathbf{w}^{(k-1)}_{i,e-2})$ to and subtracting $F_i(\mathbf{w}^{(k-1)^\star}_i)$ from both hand sides of the above inequality results in the following bound:
 \begin{equation}
     \begin{aligned}
        \mathbb{E}_{e-2} [F_i(\mathbf{w}^{(k-1)}_{i,e-1})]-F_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \left({L\mu\eta_i^2} -2\eta_i\mu+1\right) \left(F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right) 
     +\frac{L\eta_i^2}{2}\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
 \end{equation}
 Recursively expanding this expression up to the time of previous global aggregation, we get:
 \begin{equation}
     \begin{aligned}
        \mathbb{E} [F_i(\mathbf{w}^{(k-1)}_{i,E})]-F_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \left(\underbrace{{L\mu\eta_i^2} -2\eta_i\mu+1}_{\triangleq \Psi_i}\right)^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\&
     +\underbrace{\frac{L\eta_i^2}{2}\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}}_{\triangleq \varrho_i} \sum_{j=0}^{E-1}\left({L\mu\eta_i^2} -2\eta_i\mu+1\right)^j,
     \end{aligned}
 \end{equation}
 which is equivalent to:
 \begin{equation}
     \begin{aligned}
        \mathbb{E} [F_i(\mathbf{w}^{(k-1)}_{i,E})]-F_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
 Consider the global function as follows (for simplicity the number of data points are assumed to be the same for now!):
 \begin{equation}
    F(\mathbf{w}^{(k)})= \frac{1}{N} \sum_{i \in \mathcal{N}}  F_{n}(\textbf{w}^{(k)}),
\end{equation}
we have:
 \begin{equation}
 \hspace{-7mm}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})&= \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F(\mathbf{w}^{{(k)}^\star}) \right]\\&= \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F_i(\mathbf{w}^{{(k-1)}^\star}_{i})+F_i(\mathbf{w}^{{(k-1)}^\star}_{i})-F_i(\mathbf{w}^{{(k)}^\star}_{i})+F_i(\mathbf{w}^{{(k)}^\star}_{i})-F(\mathbf{w}^{{(k)}^\star}) \right]\\&
    \leq\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F_i(\mathbf{w}^{{(k-1)}^\star}_{i})+\Delta_i+\xi_i \right]\\&
    \leq\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i \right]\\&
    =\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)+F_i(\mathbf{w}^{(k-1)^\star})-F_i(\mathbf{w}^{(k-1)^\star})\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i \right]\\&=
     \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})-F_i(\mathbf{w}^{(k-1)^\star})\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i(1-\Psi_i^{E_i}) \right].
    \end{aligned}
    \hspace{-7mm}
\end{equation}
 Assuming the same step size among the nodes, i.e., $\Psi_i=\Psi\triangleq (1-2\eta\mu+L\eta^2\mu)$, $\forall i$, and the same epoch sizes, i.e., $E_i=E$, we have:
  \begin{equation}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})\leq
    \Psi^{E}\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right)
     +\underbrace{\frac{1}{N} \sum_{i \in \mathcal{N}} \left[\varrho_i\frac{1-\Psi^{E}}{1-\Psi}+\Delta_i+\xi_i(1-\Psi^{E})\right]}_{\triangleq \nu}.
    \end{aligned}
\end{equation}
Recursively expanding the above expression yields:
\begin{equation}
     F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})\leq
    \Psi^{E\times k}\left(F(\mathbf{w}^{(0})- F(\mathbf{w}^{(0)^\star})\right)
     +\nu \frac{1-\Psi^{E\times k}}{1-\Psi^{E}}.
\end{equation}

==> proofClean.tex <==
\begingroup
\onecolumn %%% For single column 
\appendices
\section{Theorem 1 and 2}
(currently I am assuming the nodes have the same number of datapoints for simplicity)
% \begin{equation}
%     \begin{aligned}
% \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2=\Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2
% \end{aligned}
% \end{equation}


For each local function, for $e\geq 2$ we can write the update as:
\begin{equation}
\begin{aligned}
    \mathbf{w}^{(k-1)}_{i,e-1}&=  \mathbf{w}^{(k-1)}_{i,e-2} - \frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\\
    &= \mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\underbrace{\left(\frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) \right)}_{\triangleq \epsilon_i},
    \end{aligned}
\end{equation}
Thus, we have 
\begin{equation}
    \begin{aligned}
     \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\epsilon_i}^2.
    \end{aligned}
\end{equation}
Taking the expectation form both hand sides, we get:
\begin{equation}
    \begin{aligned}
    \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&\mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\epsilon_i-\mathbf{w}_i^{(k-1)^\star}}^2\\&
    =\mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\mathbf{w}_i^{(k-1)^\star}}^2\\&
    +2\mathbb{E}_{e-2} [\epsilon_i^\top]\left(\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    -\mathbf{w}_i^{(k-1)^\star}\right) +\mathbb{E}_{e-2} \norm{\epsilon_i}^2.
    \end{aligned}
\end{equation}
Note that SGD is unbiased, i.e., $\mathbb{E}_{e-2} [\epsilon_i^\top]=0$, and thus
\begin{equation}\label{eq:39}
    \begin{aligned}
     \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&\mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\epsilon_i-\mathbf{w}_i^{(k-1)^\star}}^2\\&
    =\mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\mathbf{w}_i^{(k-1)^\star}}^2 +\mathbb{E}_{e-2} \norm{\epsilon_i}^2.
    \end{aligned}
\end{equation}
Now we turn into calculating $\mathbb{E}_{e-2}[\Vert \epsilon_i \Vert^2]$ in the above expression. At each time instant, $\mathbb{E}_{e-2}[\Vert \epsilon_i\Vert^2]$ can be expressed as follows:
\begin{equation}\label{eq:66}
\begin{aligned}
    \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\mathbb{E}_{e-2}\Big\Vert\frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta_i}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\eta_i^2\mathbb{E}_{e-2}\Big\Vert\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2.
    \end{aligned}
\end{equation}
To obtain the above expression, we use the result described in Section 2.8 of the book (Sampling:
Design and Analysis
Second Edition, written by
Sharon L. Lohr) and get:
\begin{equation}
\begin{aligned}
    \frac{1}{\eta_i^2} \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}
     \\
      &= \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{D_i}\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &= \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{1}{D^2_i} \left\Vert D_i\nabla  f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &\leq \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{(D_i-1)}{D_i} \Theta_i}{B_i(D_i-1)}=\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
\end{equation}
Replacing the above result in~\eqref{eq:39}, we get:
\begin{equation}\label{eq:42}
    \begin{aligned}
     \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&\mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\mathbf{w}_i^{(k-1)^\star}}^2 +\eta_i^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
    \end{aligned}
\end{equation}
Considering the first term on the right hand side of the above inequality, we have:
\begin{equation}\label{eq:43}
    \begin{aligned}
     \mathbb{E}_{e-2}& \norm{\mathbf{w}^{(k-1)}_{i,e-2} -  \frac{\eta_i}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\mathbf{w}^{(k-1)^\star}}^2= \norm{\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}}^2+ {\eta_i^2} \norm{\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2\\&-2{\eta_i} \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})^\top \left(\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}\right).
    \end{aligned}
\end{equation}
Since the local functions are strongly convex, we have:
\begin{equation}
\begin{aligned}
       \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})^\top \left( \mathbf{w}_i^{(k-1)^\star}-\mathbf{w}^{(k-1)}_{i,e-2}\right) &\leq F(\mathbf{w}_i^{(k-1)^\star})-F(\mathbf{w}^{(k-1)}_{i,e-2})-\frac{\mu}{2}\norm{\mathbf{w}_i^{(k-1)^\star}-\mathbf{w}^{(k-1)}_{i,e-2}}^2.
\end{aligned}
\end{equation}
Replacing the above result in~\eqref{eq:43} combined with~\eqref{eq:42} yields:
\begin{equation}\label{eq:45}
    \begin{aligned}
     \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&(1-\eta_i\mu)\norm{\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}}^2+ {\eta_i^2} \norm{\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2\\&-2{\eta_i}\left(F(\mathbf{w}^{(k-1)}_{i,e-2})-F(\mathbf{w}_i^{(k-1)^\star})\right) +\eta_i^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
    \end{aligned}
\end{equation}
Using the smoothness characteristic of the local function, we can get:
\begin{equation}
    \norm{\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2 \leq 2L (F_i(\mathbf{w}^{(k-1)}_{i,e-2})-F_i(\mathbf{w}_i^{(k-1)^\star})),
\end{equation}
replacing of which in~\eqref{eq:45} yields:
\begin{equation}\label{eq:47}
    \begin{aligned}
     \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&(1-\eta_i\mu)\norm{\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}}^2+ 2{\eta_i^2}L (F_i(\mathbf{w}^{(k-1)}_{i,e-2})-F_i(\mathbf{w}_i^{(k-1)^\star}))\\&-2{\eta_i}\left(F(\mathbf{w}^{(k-1)}_{i,e-2})-F(\mathbf{w}_i^{(k-1)^\star})\right) +\eta_i^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}
     \\&=\norm{\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}}^2+ 2{\eta_i}\left(L\eta_i -1\right) (F_i(\mathbf{w}^{(k-1)}_{i,e-2})-F_i(\mathbf{w}_i^{(k-1)^\star}))\\& +\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}
    \end{aligned}
\end{equation}
Assuming $\eta_i\leq 1/L$, we results in
\begin{equation}
    \begin{aligned}
     \mathbb{E}_{e-2} \norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&(1-\eta_i\mu)\norm{\mathbf{w}^{(k-1)}_{i,e-2} - \mathbf{w}_i^{(k-1)^\star}}^2+\eta_i^2 \left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
    \end{aligned}
\end{equation}
Noting that $\mathbf{w}^{(k-1)}_{i,0}=\mathbf{w}^{(k-1)}$, recursively expanding the above expression, we get:
\begin{equation}
    \begin{aligned}
     \mathbb{E} \norm{\mathbf{w}^{(k-1)}_{i,E_i}-\mathbf{w}_i^{(k-1)^\star}}^2 \leq&(1-\eta_i\mu)^{E_i}\norm{\mathbf{w}^{(k-1)} - \mathbf{w}_i^{(k-1)^\star}}^2+ \eta_i^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}  \sum_{j=0}^{k-1} (1-\eta_i\mu)^j\\&
     =(\underbrace{1-\eta_i\mu}_{\triangleq \Psi_i})^{E_i}\norm{\mathbf{w}^{(k-1)} - \mathbf{w}_i^{(k-1)^\star}}^2+\underbrace{\eta_i^2 \left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}}_{\triangleq \varrho_i}  \frac{1-(1-\eta_i\mu)^{E_i}}{\eta_i\mu}.
    \end{aligned}
\end{equation}

 Considering the global weight update as follows:
 
\begin{equation}\label{eq:globAgg}
    \mathbf{w}^{(k)}=\frac{1}{N}\sum_{i=1}^{N} \mathbf{w}^{(k-1)}_{i,E_i},
\end{equation}
{\color{red} we have: (if the concept drift is imposed on \textbf{global} model...)}
\begin{equation}\label{eq:globAgg}
\begin{aligned}
   \mathbb{E} &\left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2=\mathbb{E}\left\Vert \frac{1}{N}\sum_{i=1}^{N} \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2= \mathbb{E}\left\Vert \sum_{i=1}^{N}\frac{1}{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2=\frac{1}{N^2} \mathbb{E}\left\Vert \sum_{i=1}^{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2
   \\&
   \overset{}{\leq} \frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2=\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} + \mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star}+\mathbf{w}^{{(k-1)}^\star}-\mathbf{w}^{{(k)}^\star} \right\Vert^2
   \\
   &=\frac{1}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star} \right\Vert^2+ \mathbb{E}\left\Vert\mathbf{w}^{{(k-1)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2  
   \\&+2 \mathbb{E} \left[\mathbf{w}^{{(k-1)}^\star}-\mathbf{w}^{{(k)}^\star}\right]^\top \mathbb{E}\left[\mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star}\right]  \Bigg]
   \\&= \frac{1}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star} \right\Vert^2+ \mathbb{E}\left\Vert\mathbf{w}^{{(k-1)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2 \Bigg] 
   \\&\overset{(i)}{\leq} \frac{2}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star}\right\Vert^2 +\left\Vert \mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star} \right\Vert^2 \Bigg]+ \Delta^2
   \\
   &\leq \frac{2}{N}\sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} \right\Vert^2+\frac{2}{N}\sum_{i=1}^{N}\xi_i+\Delta^2 \\
   & \overset{}{\leq} \frac{2}{N}\sum_{i=1}^{N}\left[\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E_i}_i  + \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}\right]+\frac{2}{N}\sum_{i=1}^{N}\xi_i+\Delta^2 \\&=\frac{2}{N}\sum_{i=1}^{N}\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E_i}_i +\frac{2}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}\right]+\Delta^2
   \\&\overset{(ii)}{\leq} \frac{4}{N}\sum_{i=1}^{N}\left[\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2 \Psi^{E_i}_i  + \Vert \mathbf{w}^{(k-1)^\star} - \mathbf{w}^{(k-1)^\star}_i \Vert^2\Psi^{E_i}_i\right]+\frac{2}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}\right]+\Delta^2
   \\&=\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2 \underbrace{\frac{4}{N}\sum_{i=1}^{N}\Psi^{E_i}_i}_{\triangleq\Phi} +\underbrace{\frac{2}{N}\sum_{i=1}^{N}\left[\xi_i(1+2\Psi^{E_i}_i)+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}\right]+\Delta^2}_{\triangleq  \nu}.
   \end{aligned}
   \hspace{-7mm}
\end{equation}
where in (i) and (ii) we used Cauchy–Schwarz inequality
Recursively expanding the above term gives us:
\begin{equation}
    \begin{aligned}
     \mathbb{E} \left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2&\leq {\Phi^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \sum_{j=0}^{k-1}  \Phi ^{j}
     \\&={\Phi^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \frac{1-\Phi^k}{1-\Phi}.\end{aligned}
\end{equation}



{\color{red} we have: (if the concept drift is imposed on \textbf{local} models...)}
\begin{equation}\label{eq:globAgg}
\begin{aligned}
   \mathbb{E} &\left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2=\mathbb{E}\left\Vert \frac{1}{N}\sum_{i=1}^{N} \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2= \mathbb{E}\left\Vert \sum_{i=1}^{N}\frac{1}{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2=\frac{1}{N^2} \mathbb{E}\left\Vert \sum_{i=1}^{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2
   \\&
   \overset{}{\leq} \frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2=\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} + \mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}_i^{{(k)}^\star}+\mathbf{w}_i^{{(k)}^\star}-\mathbf{w}^{{(k)}^\star} \right\Vert^2
   \\
   &=\frac{1}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2+ \mathbb{E}\left\Vert\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}_i^{{(k)}^\star} \right\Vert^2  
   \\&+2 \mathbb{E} \left[\mathbf{w}_i^{{(k-1)}^\star}-\mathbf{w}_i^{{(k)}^\star}\right]^\top \mathbb{E}\left[\mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k)}^\star} -\mathbf{w}^{{(k)}^\star}\right]  \Bigg]
   \\&= \frac{1}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} +\mathbf{w}_i^{{(k)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2+ \mathbb{E}\left\Vert\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}_i^{{(k)}^\star} \right\Vert^2 \Bigg] 
   \\&\overset{(ii)}{\leq} \frac{2}{N}\sum_{i=1}^{N}\Bigg[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star}\right\Vert^2 +\left\Vert \mathbf{w}_i^{{(k)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2 +\frac{\Delta_i^2}{2}\Bigg]
   \\
   &\leq \frac{2}{N}\sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} \right\Vert^2+\frac{2}{N}\sum_{i=1}^{N}\left[\xi_i+\frac{\Delta_i^2}{2}\right] \\
   & \overset{(ii)}{\leq} \frac{2}{N}\sum_{i=1}^{N}\left[\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E_i}_i  + \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}\right]+\frac{2}{N}\sum_{i=1}^{N}\left[\xi_i+\frac{\Delta_i^2}{2}\right] \\&=\frac{2}{N}\sum_{i=1}^{N}\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E_i}_i +\frac{2}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}+\frac{\Delta_i^2}{2}\right]
   \\&\overset{(iii)}{\leq} \frac{4}{N}\sum_{i=1}^{N}\left[\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2 \Psi^{E_i}_i  + \Vert \mathbf{w}^{(k-1)^\star} - \mathbf{w}^{(k-1)^\star}_i \Vert^2\Psi^{E_i}_i\right]+\frac{2}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}+\frac{\Delta_i^2}{2}\right]
   \\&=\mathbb{E}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2 \underbrace{\frac{4}{N}\sum_{i=1}^{N}\Psi^{E_i}_i}_{\triangleq\Phi} +\underbrace{\frac{2}{N}\sum_{i=1}^{N}\left[\xi_i(1+2\Psi^{E_i}_i)+ \varrho_i\frac{1-\Psi^{E_i}_i}{1-\Psi_i}+\frac{\Delta_i^2}{2}\right]}_{\triangleq  \nu}.
   \end{aligned}
   \hspace{-7mm}
\end{equation}
where in (i),(ii),(iii) we used Cauchy–Schwarz inequality
Recursively expanding the above term gives us:
\begin{equation}
    \begin{aligned}
     \mathbb{E} \left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2&\leq {\Phi^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \sum_{j=0}^{k-1}  \Phi ^{j}
     \\&={\Phi^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \frac{1-\Phi^k}{1-\Phi}.\end{aligned}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Theorem 3}
\input{ProofThLoss}


==> proofTh1.tex <==
\begingroup
\onecolumn %%% For single column
\begin{proof}(currently I am assuming the nodes have the same number of datapoints for simplicity)
 We start the proof by recursively expanding the local updates, which results in the following expression for the weight obtained at the last local update:
\begin{equation}
    \mathbf{w}^{(k)}_{i,E_i}= \mathbf{w}^{(k-1)}- \frac{\eta}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
\end{equation}
Consequently, the global aggregation given in~\eqref{eq:globAgg} can be written as:
\begin{equation}
    \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
\end{equation}
The above update can be expressed in terms of a centralized gradient descent update with an additional noise term as follows:
\begin{equation}\label{eq:update1}
    \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) + e^{(k)} = \mathbf{w}^{(k-1)}-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)},
\end{equation}
where the error term is given by:
\begin{equation}
    e^{(k)}=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
\end{equation}


Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
\begin{equation}\label{eq:quadBound}
 \begin{aligned}
     F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ (\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)})^\top \nabla F(\mathbf{w}^{(k-1)})+\frac{L}{2}\norm{\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)}}^2.
     \end{aligned}
 \end{equation}
 By replacing the update rule given in~\eqref{eq:update1} in the above inequality, we get:
 \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ (-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)})^\top \nabla F(\mathbf{w}^{(k-1)})
     +\frac{L}{2}\norm{-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)}}^2.
     \end{aligned}
 \end{equation}
 Performing some algebraic manipulations on the above inequality yields:
  \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})- \eta \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2 + e^{(k)^\top} \nabla F(\mathbf{w}^{(k-1)})\\&
     +\frac{L}{2}\left(\eta^2\Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2+\Vert e^{(k)}\Vert^2-2\eta e^{(k)^\top}\nabla F(\mathbf{w}^{(k-1)})\right).
     \end{aligned}
 \end{equation}
 Thus, we have:
 \begin{equation}
     \begin{aligned}
         F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2 + \left(1-L\eta \right)e^{(k)^\top} \nabla F(\mathbf{w}^{(k-1)})
     +\frac{L}{2}\Vert e^{(k)}\Vert^2.
     \end{aligned}
 \end{equation}
 For a given weight spread at the beginning of the $k$-th global aggregation among the devices, i.e., $\mathbf{w}^{(k-1)}$, we take the expectation from the both hand sides of the above inequality, which yields:
 \begin{equation}\label{eq:49}
 \hspace{-5mm}
     \begin{aligned}
         \mathbb{E}_{k-1} [F(\mathbf{w}^{(k)})]\leq& F(\mathbf{w}^{(k-1)})+ \underbrace{ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2}_{(a)} + \underbrace{\left(1-L\eta \right)\mathbb{E}_{k-1}[e^{(k)^\top}] \nabla F(\mathbf{w}^{(k-1)})}_{(b)}
     +\underbrace{\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]}_{(c)}.
     \end{aligned}
     \hspace{-5mm}
 \end{equation}
 It can be seen that the above bound gives us the one step decrease of the value of the global loss function, which is what we desire. To further characterize the bound, we  carefully investigate terms (a), (b), and (c) appearing on the right hand side of the above inequality. 
 
 \textbf{Term (a) in~\eqref{eq:49}}: Starting from term (a), noting that the algorithm should work when $\eta$ is sufficiently small, the coefficient of the norm square of gradient is negative for sufficiently small step sizes. To avoid sign change in the coefficient, we 
 tune the step size such that $\frac{L\eta^2}{2} -\eta <0$, implying $\eta \leq 2/L$. As a result, to obtain an upper bound for (a), we need to find a lower bound on the norm square of the gradient. Using the strong convexity property, we have:
 \begin{equation}
        \norm{\nabla F(\mathbf{w}^{(k-1)})}^2 \geq \left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right){2\mu}.
 \end{equation}
 Thus, we get:
 \begin{equation}
     (a) \leq \mu \left({ L\eta^2} -2\eta\right)\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right).
 \end{equation}
 
 {\color{blue} We wanna maximize this term: Initial approach: \textbf{Term (b) in~\eqref{eq:49}}: For term (b), noting that the selection of the data points for each batch of SGD is conducted uniformly at random without replacement, SGD is an unbiased estimate of the true gradient. This implies the following equality:
 \begin{equation}
 \begin{aligned}
     & \mathbb E_{k-1}[ e^{(k)}]=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\mathbb E_{t-1}\left[\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\right]\\
      &=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iD_i}\sum_{e=1}^{E_i}\sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\\
      &=\eta \nabla F(\mathbf{w}^{(k-1)})- \frac{\eta}{E_i}\sum_{e=1}^{E_i}\nabla  F(\mathbf{w}^{(k-1)}_{i,e-1}),
      \end{aligned}
      \hspace{-15mm}
 \end{equation}
 based on which we get:
 \begin{equation}\label{eq:60s}
 \begin{aligned}
    &(b)=  \eta\left(1-L\eta \right) \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert^2 -\eta\left(1-L\eta \right)\frac{\sum_{e=1}^{E_i} < \nabla  F(\mathbf{w}^{(k-1)}_{i,e-1}), \nabla F(\mathbf{w}^{(k-1)})>}{E_i}.
    \end{aligned}
 \end{equation}
 Since the method should work with sufficiently small values of step size, to avoid sign changes we impose $\eta\leq 1/L$, which implies $1-L\eta \geq 0$. Noting that for any two vectors $a$, $b$, we have $-<a,b> ~\leq ||a||\times  ||b||$, \eqref{eq:60s} can be written as:
  \begin{equation}\label{eq:60s}
 \begin{aligned}
    &(b)\leq \eta\left(1-L\eta \right) \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert^2\\& +\eta\left(1-L\eta \right)\frac{\sum_{e=1}^{E_i} \Vert \nabla  F(\mathbf{w}^{(k-1)}_{i,e-1})\Vert \times \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert}{E_i}\\&
    \leq \eta\left(1-L\eta \right) L^2 \Vert \mathbf{w}^{(k-1)} - \mathbf{w}^{{(k-1)}^\star}\Vert^2\\& +\eta\left(1-L\eta \right)\frac{L^2\sum_{e=1}^{E_i} \Vert   \mathbf{w}^{(k-1)}_{i,e-1} -\mathbf{w}^{{(k-1)}^\star} \Vert \times \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{{(k-1)}^\star} \Vert}{E_i}
    \end{aligned}
 \end{equation}
 We leave this expression here and get back to it later in the proof. (TO DO!)}
 
 \textbf{Term (c) in~\eqref{eq:49}}: This term is given by:
 \begin{equation}\label{52}
     \begin{aligned}
    & (c)=\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]=\frac{L}{2}\mathbb{E}_{k-1} \Big\Vert\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\ 
     &
     =\frac{L}{2} \frac{\eta^2}{N^2} \mathbb{E}_{k-1}\Big\Vert\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 
     \\&
     \leq \frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 .
     \end{aligned}
 \end{equation}
 The last inequality is a result of Cauchy–Schwarz inequality, desribed by $<\textbf{a},\textbf{a}'>~\leq \norm{\textbf{a}}.\norm{\textbf{a}'}$, which results in the following bound, where $\mathbf{q}=[q_1,\cdots,q_b]$:
\begin{equation}
\begin{aligned}
    &\left(\sum_{a=1}^{b} q_i \right)^2= \left(<\mathbf{1},\mathbf{q}> \right)^2
    \leq b \sum_{a=1}^{b} q^2_i.
    \end{aligned}
\end{equation} 
The next step is to further bound~\eqref{52}. We take the following steps:
\begin{equation}\label{eq:54}
    \begin{aligned}
        &\frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\
        &\overset{(i)}{=}\frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Bigg\Vert\left(\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\right)\\
        &- \left(\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \right) \Bigg\Vert^2\\
        &\overset{(ii)}{\leq} \frac{{L}\eta^2}{N}\sum_{i=1}^{N} \underbrace{\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d)} \\
        &+\frac{{L}\eta^2}{N}\sum_{i=1}^{N}\underbrace{\mathbb{E}_{k-1} \Bigg\Vert\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})  \Bigg\Vert^2}_{(e)},
    \end{aligned}
    \hspace{-10mm}
\end{equation}
where in (i) we have added and subtracted the same term inside the norm and (ii) is the result of Cauchy–Schwarz inequality  described above. Now, we focus on each of these terms and try to further bound them:
\begin{equation}\label{eq:55}
    \begin{aligned}
        (d) &=\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
        =\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{E_i}\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
        =\frac{1}{E^2_i}\mathbb{E}_{k-1}\Bigg\Vert\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
        \leq \frac{1}{E_i}\mathbb{E}_{k-1}\sum_{e=1}^{E_i} \underbrace{\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d')},
    \end{aligned}
\end{equation}
where the last inequality is the result of Cauchy–Schwarz inequality  described above. Now, the above equation, resembles a known result in sampling theory. In $(d')$, the first term inside the norm is the \textit{true average of a population} and the second term is the \textit{sampled average of a population}. Thus, the last result of~\eqref{eq:55} can be considered as average of $E_i$ trail of variance of uniform sampling without replacement.
We can use the result described in Section 2.8 of the book (Sampling:
Design and Analysis
Second Edition, written by
Sharon L. Lohr). Using that result, we get:

\begin{equation}
    (d')= \left(1-\frac{B_i}{D_i}\right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) - \nabla F_i (\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)} ,
\end{equation}
 and thus
\begin{equation}
\begin{aligned}
    (d)&\leq \left( 1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)}.
    \end{aligned}
\end{equation}
This result has two implications: (i) it shows that if the size of mini-batch $B_i$ is equal to the size of the local data set, i.e., $B_i=D_i$, the error vanishes, and (ii) it shows that the error is a function of internal heterogeneity of the local dataset. 

Now, we turn into bounding the term (e). Term (e) corresponds to the error between (i) sequentially applying the SGD to the batches of data and where the SGD uses the result of the previous batch as the initial point for the next batch, and (ii) the case where the data is partitioned into different batches and the SGD is applied to all of the batches using the same initial points across the batches. We get:
 \begin{equation}\label{eq:57}
     \begin{aligned}
     (e)&= \mathbb{E}_{k-1} \Bigg\Vert \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
     = \frac{1}{\left(E_iB_i\right)^2}\mathbb{E}_{k-1}  \Bigg\Vert \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
     \overset{(i)}{\leq}\frac{1}{E_iB_i} \mathbb{E}_{k-1} \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \Big\Vert  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Big\Vert^2\\&
      \overset{(ii)}{\leq} \frac{L^2}{E_i} \mathbb{E}_{k-1}\sum_{e=1}^{E_i}  \Big\Vert  \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)} \Big\Vert^2,
     \end{aligned}
 \end{equation}
where in (i) we used the Cauchy–Schwarz inequality as described previously, and (ii) is due to L-smoothness. The last term can be interpreted as conducting SGD on local dataset for $E_i$ epochs of minibatch size $B_i$ and then calculating the cumulative average squared error.

For each local function, for $e\geq 2$ we can write the update as:
\begin{equation}
\begin{aligned}
    \mathbf{w}^{(k-1)}_{i,e-1}&=  \mathbf{w}^{(k-1)}_{i,e-2} - \frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\\
    &= \mathbf{w}^{(k)}_{i,e-2} -  \frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\underbrace{\left(\frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) \right)}_{\triangleq \epsilon_i},
    \end{aligned}
\end{equation}
In the above format, the local updates are written in terms of conducting a full batch GD with an added noise that is due to the minibatch SGD. Since the local functions are smooth, we have:
Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
\begin{equation}\label{eq:quadBound}
 \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})+ (\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2})^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})+\frac{L}{2}\norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2}}^2.
     \end{aligned}
 \end{equation}
 Consequently, we have:
 \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})+ (-\eta\nabla F(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i)^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\norm{-\eta\nabla F(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i}^2.
     \end{aligned}
 \end{equation}
 Performing some algebraic manipulations on the above inequality yields:
  \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})- \eta \Vert\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \epsilon_i^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\\&
     +\frac{L}{2}\left(\eta^2\Vert\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2+\Vert \epsilon_i\Vert^2-2\eta \epsilon_i^\top\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\right).
     \end{aligned}
 \end{equation}
 Thus, we get:
 \begin{equation}\label{eq:59}
     \begin{aligned}
         f_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \left(1-L\eta \right)\epsilon_i^{\top} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
 \end{equation}
 Taking the expectation w.r.t the data sampling procedure at node $i$, since SGD is unbiased we have:
 \begin{equation}
     \mathbb{E} \left[ \frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right]=\frac{\eta}{E_iD_i}  \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}),
 \end{equation}
implying:
\begin{equation}
    \mathbb{E}[ \epsilon_i]=\eta\left(\frac{E_i-1}{E_i}\right)\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2}).
\end{equation}
Taking the expectation from both hand side of~\eqref{eq:59} and applying the above result yields:
  \begin{equation}\label{eq:62}
       \hspace{-5mm}
     \begin{aligned}
        &\mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 +\left(1-L\eta \right)\eta\left(\frac{E_i-1}{E_i}\right)\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
     \hspace{-5mm}
 \end{equation}
  To avoid sign change in the second term of the right hand side, we 
 tune the step size such that $\frac{L\eta^2}{2} -\eta <0$, implying $\eta \leq 2/L$. To achieve the same goal for the third term it is sufficient to satisfy $\eta\leq 1/L$. Using the strong convexity, we have:
 \begin{equation}
        \norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2 \geq \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right){2\mu},
 \end{equation}
 where $\mathbf{w}^{(k-1)^\star}_i$ denotes the local optimal point of the local dataset at node $i$. On the other hand, using the L-smoothness, we have:
  \begin{equation}
        \norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2=\norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})-\nabla f_i(\mathbf{w}^{(k-1)^\star}_i)}^2 \leq L^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2,
 \end{equation}
 Replacing the above two results in~\eqref{eq:62}, we get:
  \begin{equation}\label{eq:65}
     \begin{aligned}
        &\mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \mu\left({L\eta^2} -2\eta\right)  (f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)) +\\ &\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i \Vert^2.
     \end{aligned}
 \end{equation}
Now we turn into calculating $\mathbb{E}_{e-2}[\Vert \epsilon_i \Vert^2]$ in the above expression. At each time instant, $\mathbb{E}_{e-2}[\Vert \epsilon_i\Vert^2]$ can be expressed as follows:
\begin{equation}\label{eq:66}
\begin{aligned}
    \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\mathbb{E}_{e-2}\Big\Vert\frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\eta^2\mathbb{E}_{e-2}\Big\Vert\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&\overset{(i)}{=}\eta^2\mathbb{E}_{e-2}\Bigg\Vert \left(\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right) \\&+ \left(\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right)\Bigg\Vert^2
    \\&\overset{(ii)}{\leq}2\eta^2\underbrace{\mathbb{E}_{e-2}\Big\Vert \frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2}_{(ii-a)} \\&+2\eta^2 \underbrace{\mathbb{E}_{e-2}\Big\Vert\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2}_{(ii-b)},
    \end{aligned}
\end{equation}
where we added and subtracted a term in (i) to exploit the sampling characteristics of SGD and then applied Cauchy–Schwarz inequality. The two terms $(ii-a)$ and $(ii-b)$ can be obtained as follows.

To obtain $(ii-a)$, we use the result described in Section 2.8 of the book (Sampling:
Design and Analysis
Second Edition, written by
Sharon L. Lohr) and get:
\begin{equation}
    (ii-a)=\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}.
\end{equation}
To obtain $(ii-b)$, we use the characteristic of the local loss function, which implies:
\begin{equation}
\begin{aligned}
    (ii&-b)=\mathbb{E}_{e-2}\Big\Vert\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\frac{1}{B^2_i}\mathbb{E}_{e-2}\Big\Vert \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\left(\frac{E_i-1}{B_iE_i}\right)^2\mathbb{E}\Big\Vert \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2\leq\frac{(E_i-1)^2}{B_iE^2_i}\mathbb{E}\left[\sum_{b\in \mathcal{B}_{i,e-1}}\Big\Vert \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2\right]
    \\&\leq \left(\frac{E_i-1}{E_i}\right)^2 \Big\Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Big\Vert^2.
    \end{aligned}
\end{equation}
Replacing the above results in~\eqref{eq:66} yields:
\begin{equation}
    \begin{aligned}
    \mathbb{E}\Vert \epsilon \Vert^2 \leq& 2\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
    \end{aligned}
\end{equation}
Replacing the above result in~\eqref{eq:65}, we get:
  \begin{equation}\label{eq:65_1}
     \begin{aligned}
        \mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]-f_i(\mathbf{w}^{(k-1)}_{i,e-2})&\leq \mu\left({L\eta^2} -2\eta\right) \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
 Adding $f_i(\mathbf{w}^{(k-1)}_{i,e-2})$ to and subtracting $f_i(\mathbf{w}^{(k-1)^\star}_i)$ from both hand sides of the above inequality results in the following bound:
 \begin{equation}\label{eq:71}
     \begin{aligned}
        \mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]-f_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \left({L\mu\eta^2} -2\eta\mu+1\right) \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k)}_{i,e-2}- \mathbf{w}^{(k)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
Since the local function is L-smooth, we get:
\begin{equation}
    f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i) \leq \frac{L}{2} \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2,
\end{equation}
Also, since the local function is strong convex, we have:
\begin{equation}
\frac{\mu}{2}    \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2  \leq  f_i(\mathbf{w}^{(k-1)}_{i,e-1})- f_i(\mathbf{w}^{(k-1)^\star}_i).
\end{equation}
Replacing the above two results in~\eqref{eq:71} results in the following bound:
 \begin{equation}\label{eq:74}
     \begin{aligned}
        \frac{\mu}{2}    \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq& \left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
Equivalently, we have:
 \begin{equation}\label{eq:75}
     \begin{aligned}
        &   \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq\\& \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2\left( \left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} +\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)+L\eta^2\left(\frac{E_i-1}{E_i}\right)^2\right)\frac{2}{\mu}  \\&
     +\frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}.
     \end{aligned}
 \end{equation}
We define the following two quantities to simplify the above expression:
 \begin{equation}
     \begin{aligned}
       \Psi_i \triangleq \left(\left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} +\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)+L\eta^2\left(\frac{E_i-1}{E_i}\right)^2\right)\frac{2}{\mu} ,
     \end{aligned}
 \end{equation}
  \begin{equation}\label{eq:77}
     \begin{aligned}
  \theta_i( \mathbf{w}^{(k-1)}_{i,e-2})\triangleq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)},
     \end{aligned}
 \end{equation}
 where $\Theta_i( \mathbf{w}^{(k-1)}_{i,e-2})$ corresponds to diversity of data at the node. More specifically, it measures the square error of gradient evaluated at individual local datapoints. It is evident that as the distribution of local data becomes more homogeneous this quantity decreases. 
 Using Assumption~\ref{Assump:DataVariabilit}, we get:
 \begin{equation}
 \begin{aligned}
    & \theta_i( \mathbf{w}^{(k-1)}_{i,e-2})= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\
     &= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{D_i}\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{1}{D^2_i} \left\Vert D_i\nabla  f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &\leq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{(D_i-1)}{D_i} \Theta_i}{B_i(D_i-1)}=\frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
 \end{equation}
 Let $\varrho_i \triangleq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}$. By replacing the above results in~\eqref{eq:75}, we get:
 \begin{equation}\label{eq:80}
     \begin{aligned}
       \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi_i  + \varrho_i.
     \end{aligned}
 \end{equation}
 The above expression is the one step decrease of the  local function during the period of local updates. Recursively expanding the above expression, since the local iterations starts with receiving the model parameter $\mathbf{w}^{(k-1)}$ from the server, i.e., $\mathbf{w}^{(k-1)}_{i,0}=\mathbf{w}^{(k-1)}$, we get:
  \begin{equation}
     \begin{aligned}
       \mathbb{E} \Vert \mathbf{w}^{(k-1)}_{i,e}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{e}_i  + \sum_{j=0}^{e-1}\Psi^{j}_i\varrho_i,
     \end{aligned}
 \end{equation}
which is equivalent to:
  \begin{equation}\
     \begin{aligned}
       \mathbb{E} \Vert \mathbf{w}^{(k-1)}_{i,e}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{e}_i  + \varrho_i\frac{1-\Psi^{e}_i}{1-\Psi_i}, ~e\geq 1.
     \end{aligned}
 \end{equation}
 We replace this result in~\eqref{eq:57} to obtain the following result:
 \begin{equation}
 \begin{aligned}
     (e)&\leq \frac{L^2}{E_i}\mathbb{E}_{k-1}  \sum_{e=1}^{E_i}  \Bigg\Vert  \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)} \Bigg\Vert^2
     \\&\overset{(i)}{\leq} \frac{2L^2}{E_i} \mathbb{E}_{k-1}\sum_{e=1}^{E_i-1}  \left[\Big\Vert  \mathbf{w}^{(k-1)}_{i,e}-\mathbf{w}^{(k-1)^\star}_i \Big\Vert^2+ \Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2\right]\\
     &\leq \frac{2L^2}{E_i} \left(\sum_{e=1}^{E_i-1} \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{e}_i  + \varrho_i\frac{1-\Psi^{e}_i}{1-\Psi_i}\right) + 2L^2 \Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2\\
     &=\frac{2L^2}{E_i} \left( \Psi_i\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}  + \varrho_i\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}\right) + 2L^2 \Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2\\
     &=\Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2 \left(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right)+\frac{2L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
 where in (i) we used triangle and Cauchy–Schwarz inequality and the fact that $\mathbf{w}^{(k-1)}_{i,0}=\mathbf{w}^{(k-1)}$. Combining the above result with~\eqref{eq:49},~\eqref{eq:54},~\eqref{eq:55}, we get the following bound on the convergence of the global function:
 \begin{equation}
     \begin{aligned}
      \mathbb{E}_{k-1} [F(\mathbf{w}^{(k)})]\leq& F(\mathbf{w}^{(k-1)})+ \mu \left({ L\eta^2} -2\eta\right)\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right) \\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)}\\&
     +\frac{{L}\eta^2}{N}\left[\sum_{i=1}^{N}\Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2 \left(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right)+\frac{2L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}\right]\\&
     \leq F(\mathbf{w}^{(k-1)})+ \mu \left({ L\eta^2} -2\eta\right)\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right) \\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right)  \frac{ \Theta_i}{B_i}\\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N}\Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2 \left(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right)+\frac{2L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
Subtracting $F(\mathbf{w}^{(k)^\star})$ from both hand sides, results in the following bound: (stationary optimal solutions!! Concept Drift will appear here!)
\begin{equation}\label{eq:85}
     \begin{aligned}
      \mathbb{E}_{k-1} [F(\mathbf{w}^{(k)})]-F(\mathbf{w}^{(k)^\star})\leq& \left({  \mu L\eta^2} -2\eta \mu+1\right)\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k)^\star})\right) \\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right)  \frac{ \Theta_i}{B_i}\\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N}\Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2 \Bigg(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \Bigg)\\&+\frac{2L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
Since the global function is L-smooth and $\mu$ strongly convex, we have:
\begin{equation}
    F(\mathbf{w}^{(k-1)})-F(\mathbf{w}^{(k-1)^\star}) \leq \frac{L}{2} \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{(k-1)^\star} \Vert^2,
\end{equation}
Also, since the local function is strong convex, we have:
\begin{equation}
\frac{\mu}{2}    \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2  \leq  F(\mathbf{w}^{(k-1)})-F(\mathbf{w}^{(k-1)^\star}),
\end{equation}

Replacing the above two results in~\eqref{eq:85} results in the following bound:
\begin{equation}\label{eq:88}
     \begin{aligned}
      \mathbb{E}_{k-1} \frac{\mu}{2}    \Vert \mathbf{w}^{(k)}- \mathbf{w}^{(k)^\star} \Vert^2\leq &\left({  \mu L\eta^2} -2\eta \mu+1\right)\frac{L}{2} \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{(k)^\star} \Vert^2 \\&
      +\frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right)  \frac{ \Theta_i}{B_i}\\&
     +\frac{{L}\eta^2}{N}\sum_{i=1}^{N}\Big\Vert\mathbf{w}^{(k-1)^\star}_i- \mathbf{w}^{(k-1)} \Big\Vert^2 \Bigg(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \Bigg)\\&+\frac{2L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
Using the assumption on local model divergence in~\eqref{eq:88} and performing some algebraic manipulations yield:
\begin{equation}\label{eq:90}
    \begin{aligned}
      \mathbb{E}_{k-1}  \Vert \mathbf{w}^{(k)}- \mathbf{w}^{(k)^\star} \Vert^2\leq& \frac{L}{\mu}   \left({  \mu L\eta^2} -2\eta \mu+1\right) \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{(k)^\star} \Vert^2 \\&
     +\frac{2}{\mu} \frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right)  \frac{ \Theta_i}{B_i}\\&
     +\frac{2}{\mu} \frac{{L}\eta^2}{N}\sum_{i=1}^{N}2\left(\Big\Vert\mathbf{w}^{(k)^\star}- \mathbf{w}^{(k-1)} \Big\Vert^2 +\xi_i\right) \left(\frac{2L^2\Psi_i}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right)\\&+\frac{4}{\mu} \frac{L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
     \end{aligned}
\end{equation}
To simplify the above expression, we define the following quantities:
\begin{equation}
    \alpha\triangleq \frac{L}{\mu}   \left({  \mu L\eta^2} -2\eta \mu+1\right),
\end{equation}
\begin{equation}
    \Xi\triangleq \frac{2}{\mu} \frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left( 1-\frac{B_i}{D_i} \right)  \frac{ \Theta_i}{B_i},
\end{equation}
\begin{equation}
    \chi\triangleq \frac{4}{\mu} \frac{{L}\eta^2}{N}\sum_{i=1}^{N} \left(\frac{2L^2}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right),
\end{equation}
\begin{equation}
    \Phi \triangleq \frac{4}{\mu} \frac{{L}\eta^2}{N}\sum_{i=1}^{N}\xi_i \left(\frac{2L^2}{E_i}\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}+2L^2 \right)+\frac{4}{\mu} \frac{L^2\varrho_i}{E_i}\frac{E_i-\Psi_i\frac{1-\Psi^{E_i-1}_i}{1-\Psi_i}}{1-\Psi_i}.
\end{equation}
Consequently, the bound in~\eqref{eq:90} can be written as:
\begin{equation}\label{eq:95}
    \begin{aligned}
      &\mathbb{E}_{k-1}  \Vert \mathbf{w}^{(k)}- \mathbf{w}^{(k)^\star} \Vert^2\leq (\alpha+\chi)\Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{(k)^\star} \Vert^2 + \Xi+\Phi.
     \end{aligned}
\end{equation}
Assuming that the local and global optimal solution remains constant over time (concept drift accumulates here!!), recursively expanding the above term results in the following upper bound of convergence of the global loss function:
\begin{equation}\label{eq:96}
      \begin{aligned}
      &\mathbb{E} \Vert \mathbf{w}^{(k)}- \mathbf{w}^{(k)^\star} \Vert^2\leq (\alpha+\chi)^{(k)} \Vert \mathbf{w}^{0}-\mathbf{w}^{(k)^\star} \Vert^2 + \frac{1-(\alpha+\chi)^{(k)}}{1-(\alpha+\chi)}\left(\Xi+\Phi\right).
     \end{aligned}
\end{equation}
\end{proof}
Next week: Extension to model drift case where the local and global optimal solutions start drifting over time.

% --------------------------------------------------------

% We then use the result described in Section 2.8 of the book (Sampling:
% Design and Analysis
% Second Edition, written by
% Sharon L. Lohr) and get:
% \begin{equation}\label{eq:63}
% \begin{aligned}
%     \frac{L}{2} \mathbb{E}[\Vert e^{(k)}\Vert^2]&\leq \frac{L}{2} \frac{1}{E_i} \left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)}\triangleq \Xi^t.
%     \end{aligned}
% \end{equation}
% From the above discussion, we can get (there are a lot of abuse of notations here specially due to the time index, I need to revise the time index above):
% \begin{equation}
% \begin{aligned}
%   E[f_i({w}^t_{i,e-1})-f_i(\mathbf{w}^{(k)}_{i,e-2}) ]\leq& \mu \left({ L\eta^2} -2\eta\right)(f_i(\mathbf{w}^{(k)}_{i,e-2})- f_i(\mathbf{w}^{(k)^\star}))
%      +\Xi^t,~~ \forall t.
%     \end{aligned}
% \end{equation}
% After some modifications and algebraic manipulations, we get:
% \begin{equation}\label{here}
% \begin{aligned}
%   E[f_i({w}^t_{i,e-1})-f_i(\mathbf{w}^{(k)^\star}) ]\leq& A \left(1-\eta \mu \right)^{e-1}(f_i(\mathbf{w}^{(k-1)}- f_i(\mathbf{w}^{(k)^\star}))
%      +B\sum_{m=1}^{e-1}\left(1-\eta \mu \right)^t \Xi^t,~~ \forall t,
%     \end{aligned}
% \end{equation}
% where $A$ and $B$ are going to be derived later.
% Finally, to obtain (e), we use the strong convexity of the local functions that implies the following inequality:
% \begin{equation}
% \begin{aligned}
%   &\mathbb{E}_{k-1} ||\mathbf{w}^{(k)}_{i,e-1}-\mathbf{w}^{(k-1)}||^2\leq \mathbb{E}_{k-1} ||\mathbf{w}^{(k)}_{i,e-1}-\mathbf{w}^{(k)^\star} -\mathbf{w}^{(k-1)}+\mathbf{w}^{(k)^\star}||^2\\&
%   \leq  \mathbb{E}_{k-1}\left( ||\mathbf{w}^{(k)}_{i,e-1}-\mathbf{w}^{(k)^\star}|| + || \mathbf{w}^{(k-1)}-\mathbf{w}^{(k)^\star}||\right)^2 \\&
%   \leq 2 \mathbb{E}_{k-1} ||\mathbf{w}^{(k)}_{i,e-1}-\mathbf{w}^{(k)^\star}||^2 + 2 \mathbb{E}_{k-1}|| \mathbf{w}^{(k-1)}-\mathbf{w}^{(k)^\star}||^2
%     \end{aligned}
% \end{equation}
% where in the last step we applied Cauchy–Schwarz inequality.
% Then, we use the strong convexity of the local functions that implies the following inequality:
% \begin{equation}
%     \mathbb{E}_{k-1}\frac{\mu}{2}|| \mathbf{w}^{(k)}_{i,e-1}-\mathbf{w}^{(k)^\star} || \leq \mathbb{E}_{k-1} [f_i(\mathbf{w}^{(k)}_{i,e-1})-f(\mathbf{w}^{(k-1)})],
% \end{equation}
% Thus, where the right hand side of the above inequality is given in~\eqref{here}. Note that there is one term that remains in the derivations and that is the variability of data at the node that also appears in the right hand side of~\eqref{eq:63}. In the following, we propose one approach to bound data variability. 

% To bound data variability, it is sufficient to bound the following term \\$\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2$, which can be bounded as follows using Cauchy–Schwarz inequality:
% \begin{equation*}
%     \sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2\leq 2\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\right\Vert^2 +2\sum_{b=1}^{D_i}\left\Vert \nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2 \triangleq \Phi^{t-1}_i
% \end{equation*}
% Using L-smoothness of the local and global function, we have:
% \begin{equation}
% \begin{aligned}
%     \Phi^{t-1}_i \leq& 4\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-f_i(\mathbf{w}^{{(k-1)}^\star}_i,x_{i,b})\right\Vert^2 + 4\sum_{b=1}^{D_i} ||f_i(\mathbf{w}^{{(k-1)}^\star}_i,x_{i,b})||^2\\&+ 2L^2 D_i \Vert \mathbf{w}^{(k-1)}-w_i^{{t-1}^\star} \Vert^2,
%     \end{aligned}
% \end{equation}
% where $\mathbf{w}^{{(k-1)}^\star}_i$ denotes the instantaneous optimal model for the local dataset at node $i$ (note that due to model drift, this parameter can vary over time). The interesting fact about the above inequality is that it connects the data variability to the distance of the global model from the local optimal solution. Next week I will redo all the above steps to see whether we can find a better approach to bound them.

==> proofTh1_withoutGlobal.tex <==
\begingroup
\onecolumn %%% For single column
\begin{proof}(currently I am assuming the nodes have the same number of datapoints for simplicity)
%  We start the proof by recursively expanding the local updates, which results in the following expression for the weight obtained at the last local update:
% \begin{equation}
%     \mathbf{w}^{(k-1)}_{i,E_i}= \mathbf{w}^{(k-1)}- \frac{\eta}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}
% Consequently, the global aggregation given in~\eqref{eq:globAgg} can be written as:
% \begin{equation}
%     \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}
% The above update can be expressed in terms of a centralized gradient descent update with an additional noise term as follows:
% \begin{equation}\label{eq:update1}
%     \mathbf{w}^{(k)}=\mathbf{w}^{(k-1)}-\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) + e^{(k)} = \mathbf{w}^{(k-1)}-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)},
% \end{equation}
% where the error term is given by:
% \begin{equation}
%     e^{(k)}=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}).
% \end{equation}


% Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
% \begin{equation}\label{eq:quadBound}
%  \begin{aligned}
%      F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ (\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)})^\top \nabla F(\mathbf{w}^{(k-1)})+\frac{L}{2}\norm{\mathbf{w}^{(k)}-\mathbf{w}^{(k-1)}}^2.
%      \end{aligned}
%  \end{equation}
%  By replacing the update rule given in~\eqref{eq:update1} in the above inequality, we get:
%  \begin{equation}
%       \begin{aligned}
%      F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ (-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)})^\top \nabla F(\mathbf{w}^{(k-1)})
%      +\frac{L}{2}\norm{-\eta\nabla F(\mathbf{w}^{(k-1)}) + e^{(k)}}^2.
%      \end{aligned}
%  \end{equation}
%  Performing some algebraic manipulations on the above inequality yields:
%   \begin{equation}
%       \begin{aligned}
%      F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})- \eta \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2 + e^{(k)^\top} \nabla F(\mathbf{w}^{(k-1)})\\&
%      +\frac{L}{2}\left(\eta^2\Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2+\Vert e^{(k)}\Vert^2-2\eta e^{(k)^\top}\nabla F(\mathbf{w}^{(k-1)})\right).
%      \end{aligned}
%  \end{equation}
%  Thus, we have:
%  \begin{equation}
%      \begin{aligned}
%          F(\mathbf{w}^{(k)})\leq& F(\mathbf{w}^{(k-1)})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2 + \left(1-L\eta \right)e^{(k)^\top} \nabla F(\mathbf{w}^{(k-1)})
%      +\frac{L}{2}\Vert e^{(k)}\Vert^2.
%      \end{aligned}
%  \end{equation}
%  For a given weight spread at the beginning of the $k$-th global aggregation among the devices, i.e., $\mathbf{w}^{(k-1)}$, we take the expectation from the both hand sides of the above inequality, which yields:
%  \begin{equation}\label{eq:49}
%  \hspace{-5mm}
%      \begin{aligned}
%          \mathbb{E}_{k-1} [F(\mathbf{w}^{(k)})]\leq& F(\mathbf{w}^{(k-1)})+ \underbrace{ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla F(\mathbf{w}^{(k-1)})\Vert^2}_{(a)} + \underbrace{\left(1-L\eta \right)\mathbb{E}_{k-1}[e^{(k)^\top}] \nabla F(\mathbf{w}^{(k-1)})}_{(b)}
%      +\underbrace{\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]}_{(c)}.
%      \end{aligned}
%      \hspace{-5mm}
%  \end{equation}
%  It can be seen that the above bound gives us the one step decrease of the value of the global loss function, which is what we desire. To further characterize the bound, we  carefully investigate terms (a), (b), and (c) appearing on the right hand side of the above inequality. 
 
%  \textbf{Term (a) in~\eqref{eq:49}}: Starting from term (a), noting that the algorithm should work when $\eta$ is sufficiently small, the coefficient of the norm square of gradient is negative for sufficiently small step sizes. To avoid sign change in the coefficient, we 
%  tune the step size such that $\frac{L\eta^2}{2} -\eta <0$, implying $\eta \leq 2/L$. As a result, to obtain an upper bound for (a), we need to find a lower bound on the norm square of the gradient. Using the strong convexity property, we have:
%  \begin{equation}
%         \norm{\nabla F(\mathbf{w}^{(k-1)})}^2 \geq \left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right){2\mu}.
%  \end{equation}
%  Thus, we get:
%  \begin{equation}
%      (a) \leq \mu \left({ L\eta^2} -2\eta\right)\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right).
%  \end{equation}
 
%  {\color{blue} We wanna maximize this term: Initial approach: \textbf{Term (b) in~\eqref{eq:49}}: For term (b), noting that the selection of the data points for each batch of SGD is conducted uniformly at random without replacement, SGD is an unbiased estimate of the true gradient. This implies the following equality:
%  \begin{equation}
%  \begin{aligned}
%      & \mathbb E_{k-1}[ e^{(k)}]=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\mathbb E_{t-1}\left[\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\right]\\
%       &=\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iD_i}\sum_{e=1}^{E_i}\sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})\\
%       &=\eta \nabla F(\mathbf{w}^{(k-1)})- \frac{\eta}{E_i}\sum_{e=1}^{E_i}\nabla  F(\mathbf{w}^{(k-1)}_{i,e-1}),
%       \end{aligned}
%       \hspace{-15mm}
%  \end{equation}
%  based on which we get:
%  \begin{equation}\label{eq:60s}
%  \begin{aligned}
%     &(b)=  \eta\left(1-L\eta \right) \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert^2 -\eta\left(1-L\eta \right)\frac{\sum_{e=1}^{E_i} < \nabla  F(\mathbf{w}^{(k-1)}_{i,e-1}), \nabla F(\mathbf{w}^{(k-1)})>}{E_i}.
%     \end{aligned}
%  \end{equation}
%  Since the method should work with sufficiently small values of step size, to avoid sign changes we impose $\eta\leq 1/L$, which implies $1-L\eta \geq 0$. Noting that for any two vectors $a$, $b$, we have $-<a,b> ~\leq ||a||\times  ||b||$, \eqref{eq:60s} can be written as:
%   \begin{equation}\label{eq:60s}
%  \begin{aligned}
%     &(b)\leq \eta\left(1-L\eta \right) \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert^2\\& +\eta\left(1-L\eta \right)\frac{\sum_{e=1}^{E_i} \Vert \nabla  F(\mathbf{w}^{(k-1)}_{i,e-1})\Vert \times \Vert \nabla F(\mathbf{w}^{(k-1)})\Vert}{E_i}\\&
%     \leq \eta\left(1-L\eta \right) L^2 \Vert \mathbf{w}^{(k-1)} - \mathbf{w}^{{(k-1)}^\star}\Vert^2\\& +\eta\left(1-L\eta \right)\frac{L^2\sum_{e=1}^{E_i} \Vert   \mathbf{w}^{(k-1)}_{i,e-1} -\mathbf{w}^{{(k-1)}^\star} \Vert \times \Vert \mathbf{w}^{(k-1)}-\mathbf{w}^{{(k-1)}^\star} \Vert}{E_i}
%     \end{aligned}
%  \end{equation}
%  We leave this expression here and get back to it later in the proof. (TO DO!)}
 
%  \textbf{Term (c) in~\eqref{eq:49}}: This term is given by:
%  \begin{equation}\label{52}
%      \begin{aligned}
%     & (c)=\frac{L}{2}\mathbb{E}_{k-1}[\Vert e^{(k)}\Vert^2]=\frac{L}{2}\mathbb{E}_{k-1} \Big\Vert\frac{\eta}{N}\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\frac{\eta}{N}\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\ 
%      &
%      =\frac{L}{2} \frac{\eta^2}{N^2} \mathbb{E}_{k-1}\Big\Vert\sum_{i=1}^{N}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})-\sum_{i=1}^{N} \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 
%      \\&
%      \leq \frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2 .
%      \end{aligned}
%  \end{equation}
%  The last inequality is a result of Cauchy–Schwarz inequality, desribed by $<\textbf{a},\textbf{a}'>~\leq \norm{\textbf{a}}.\norm{\textbf{a}'}$, which results in the following bound, where $\mathbf{q}=[q_1,\cdots,q_b]$:
% \begin{equation}
% \begin{aligned}
%     &\left(\sum_{a=1}^{b} q_i \right)^2= \left(<\mathbf{1},\mathbf{q}> \right)^2
%     \leq b \sum_{a=1}^{b} q^2_i.
%     \end{aligned}
% \end{equation} 
% The next step is to further bound~\eqref{52}. We take the following steps:
% \begin{equation}\label{eq:54}
%     \begin{aligned}
%         &\frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Big\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})- \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b}) \Big\Vert^2\\
%         &\overset{(i)}{=}\frac{L}{2} \frac{\eta^2}{N}\sum_{i=1}^{N} \mathbb{E}_{k-1}\Bigg\Vert\left(\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\right)\\
%         &- \left(\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \right) \Bigg\Vert^2\\
%         &\overset{(ii)}{\leq} \frac{{L}\eta^2}{N}\sum_{i=1}^{N} \underbrace{\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d)} \\
%         &+\frac{{L}\eta^2}{N}\sum_{i=1}^{N}\underbrace{\mathbb{E}_{k-1} \Bigg\Vert\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})  \Bigg\Vert^2}_{(e)},
%     \end{aligned}
%     \hspace{-10mm}
% \end{equation}
% where in (i) we have added and subtracted the same term inside the norm and (ii) is the result of Cauchy–Schwarz inequality  described above. Now, we focus on each of these terms and try to further bound them:
% \begin{equation}\label{eq:55}
%     \begin{aligned}
%         (d) &=\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         =\mathbb{E}_{k-1}\Bigg\Vert\frac{1}{E_i}\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         =\frac{1}{E^2_i}\mathbb{E}_{k-1}\Bigg\Vert\sum_{e=1}^{E_i}\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2\\&
%         \leq \frac{1}{E_i}\mathbb{E}_{k-1}\sum_{e=1}^{E_i} \underbrace{\Bigg\Vert\frac{1}{D_i}\sum_{b=1}^{D_i}\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\frac{1}{B_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b})\Bigg\Vert^2}_{(d')},
%     \end{aligned}
% \end{equation}
% where the last inequality is the result of Cauchy–Schwarz inequality  described above. Now, the above equation, resembles a known result in sampling theory. In $(d')$, the first term inside the norm is the \textit{true average of a population} and the second term is the \textit{sampled average of a population}. Thus, the last result of~\eqref{eq:55} can be considered as average of $E_i$ trail of variance of uniform sampling without replacement.
% We can use the result described in Section 2.8 of the book (Sampling:
% Design and Analysis
% Second Edition, written by
% Sharon L. Lohr). Using that result, we get:

% \begin{equation}
%     (d')= \left(1-\frac{B_i}{D_i}\right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) - \nabla F_i (\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)} ,
% \end{equation}
%  and thus
% \begin{equation}
% \begin{aligned}
%     (d)&\leq \left( 1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)})\right\Vert^2}{B_i(D_i-1)}.
%     \end{aligned}
% \end{equation}
% This result has two implications: (i) it shows that if the size of mini-batch $B_i$ is equal to the size of the local data set, i.e., $B_i=D_i$, the error vanishes, and (ii) it shows that the error is a function of internal heterogeneity of the local dataset. 

% Now, we turn into bounding the term (e). Term (e) corresponds to the error between (i) sequentially applying the SGD to the batches of data and where the SGD uses the result of the previous batch as the initial point for the next batch, and (ii) the case where the data is partitioned into different batches and the SGD is applied to all of the batches using the same initial points across the batches. We get:
%  \begin{equation}\label{eq:57}
%      \begin{aligned}
%      (e)&= \mathbb{E}_{k-1} \Bigg\Vert \frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})-\frac{1}{E_iB_i}\sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
%      = \frac{1}{\left(E_iB_i\right)^2}\mathbb{E}_{k-1}  \Bigg\Vert \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}} \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Bigg\Vert^2\\&
%      \overset{(i)}{\leq}\frac{1}{E_iB_i} \mathbb{E}_{k-1} \sum_{e=1}^{E_i}\sum_{b\in \mathcal{B}_{i,e}}  \Big\Vert  \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-1},x_{i,b})- \nabla f_i(\mathbf{w}^{(k-1)},x_{i,b}) \Big\Vert^2\\&
%       \overset{(ii)}{\leq} \frac{L^2}{E_i} \mathbb{E}_{k-1}\sum_{e=1}^{E_i}  \Big\Vert  \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)} \Big\Vert^2,
%      \end{aligned}
%  \end{equation}
% where in (i) we used the Cauchy–Schwarz inequality as described previously, and (ii) is due to L-smoothness. The last term can be interpreted as conducting SGD on local dataset for $E_i$ epochs of minibatch size $B_i$ and then calculating the cumulative average squared error.

For each local function, for $e\geq 2$ we can write the update as:
\begin{equation}
\begin{aligned}
    \mathbf{w}^{(k-1)}_{i,e-1}&=  \mathbf{w}^{(k-1)}_{i,e-2} - \frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\\
    &= \mathbf{w}^{(k)}_{i,e-2} -  \frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})
    +\underbrace{\left(\frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) \right)}_{\triangleq \epsilon_i},
    \end{aligned}
\end{equation}
In the above format, the local updates are written in terms of conducting a full batch GD with an added noise that is due to the minibatch SGD. Since the local functions are smooth, we have:
Since the global loss function is L-smooth, using the first order Taylor expansion, we get:
\begin{equation}\label{eq:quadBound}
 \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})+ (\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2})^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})+\frac{L}{2}\norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2}}^2.
     \end{aligned}
 \end{equation}
 Consequently, we have:
 \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})+ (-\eta\nabla F(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i)^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\norm{-\eta\nabla F(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i}^2.
     \end{aligned}
 \end{equation}
 Performing some algebraic manipulations on the above inequality yields:
  \begin{equation}
      \begin{aligned}
     F(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F(\mathbf{w}^{(k-1)}_{i,e-2})- \eta \Vert\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \epsilon_i^\top \nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\\&
     +\frac{L}{2}\left(\eta^2\Vert\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2+\Vert \epsilon_i\Vert^2-2\eta \epsilon_i^\top\nabla F(\mathbf{w}^{(k-1)}_{i,e-2})\right).
     \end{aligned}
 \end{equation}
 Thus, we get:
 \begin{equation}\label{eq:59}
     \begin{aligned}
         f_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \left(1-L\eta \right)\epsilon_i^{\top} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
 \end{equation}
 Taking the expectation w.r.t the data sampling procedure at node $i$, since SGD is unbiased we have:
 \begin{equation}
     \mathbb{E} \left[ \frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right]=\frac{\eta}{E_iD_i}  \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}),
 \end{equation}
implying:
\begin{equation}
    \mathbb{E}[ \epsilon_i]=\eta\left(\frac{E_i-1}{E_i}\right)\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2}).
\end{equation}
Taking the expectation from both hand side of~\eqref{eq:59} and applying the above result yields:
  \begin{equation}\label{eq:62}
       \hspace{-5mm}
     \begin{aligned}
        &\mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\eta^2}{2} -\eta\right) \Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 +\left(1-L\eta \right)\eta\left(\frac{E_i-1}{E_i}\right)\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
     \hspace{-5mm}
 \end{equation}
  To avoid sign change in the second term of the right hand side, we 
 tune the step size such that $\frac{L\eta^2}{2} -\eta <0$, implying $\eta \leq 2/L$. To achieve the same goal for the third term it is sufficient to satisfy $\eta\leq 1/L$. Using the strong convexity, we have:
 \begin{equation}
        \norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2 \geq \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right){2\mu},
 \end{equation}
 where $\mathbf{w}^{(k-1)^\star}_i$ denotes the local optimal point of the local dataset at node $i$. On the other hand, using the L-smoothness, we have:
  \begin{equation}
        \norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2=\norm{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2})-\nabla f_i(\mathbf{w}^{(k-1)^\star}_i)}^2 \leq L^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2,
 \end{equation}
 Replacing the above two results in~\eqref{eq:62}, we get:
  \begin{equation}\label{eq:65}
     \begin{aligned}
        &\mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq f_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \mu\left({L\eta^2} -2\eta\right)  (f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)) +\\ &\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2
     +\frac{L}{2}\mathbb{E}_{e-2}\Vert \epsilon_i \Vert^2.
     \end{aligned}
 \end{equation}
Now we turn into calculating $\mathbb{E}_{e-2}[\Vert \epsilon_i \Vert^2]$ in the above expression. At each time instant, $\mathbb{E}_{e-2}[\Vert \epsilon_i\Vert^2]$ can be expressed as follows:
\begin{equation}\label{eq:66}
\begin{aligned}
    \mathbb{E}_{e-2}\Vert \epsilon_i\Vert^2&=\mathbb{E}_{e-2}\Big\Vert\frac{\eta}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{\eta}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\eta^2\mathbb{E}_{e-2}\Big\Vert\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&\overset{(i)}{=}\eta^2\mathbb{E}_{e-2}\Bigg\Vert \left(\frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right) \\&+ \left(\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\right)\Bigg\Vert^2
    \\&\overset{(ii)}{\leq}2\eta^2\underbrace{\mathbb{E}_{e-2}\Big\Vert \frac{1}{D_i} \sum_{b=1}^{D_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2}_{(ii-a)} \\&+2\eta^2 \underbrace{\mathbb{E}_{e-2}\Big\Vert\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2}_{(ii-b)},
    \end{aligned}
\end{equation}
where we added and subtracted a term in (i) to exploit the sampling characteristics of SGD and then applied Cauchy–Schwarz inequality. The two terms $(ii-a)$ and $(ii-b)$ can be obtained as follows.

To obtain $(ii-a)$, we use the result described in Section 2.8 of the book (Sampling:
Design and Analysis
Second Edition, written by
Sharon L. Lohr) and get:
\begin{equation}
    (ii-a)=\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}.
\end{equation}
To obtain $(ii-b)$, we use the characteristic of the local loss function, which implies:
\begin{equation}
\begin{aligned}
    (ii&-b)=\mathbb{E}_{e-2}\Big\Vert\frac{1}{B_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_iB_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\frac{1}{B^2_i}\mathbb{E}_{e-2}\Big\Vert \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})-\frac{1}{E_i} \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2
    \\&=\left(\frac{E_i-1}{B_iE_i}\right)^2\mathbb{E}\Big\Vert \sum_{b\in \mathcal{B}_{i,e-1}} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2\leq\frac{(E_i-1)^2}{B_iE^2_i}\mathbb{E}\left[\sum_{b\in \mathcal{B}_{i,e-1}}\Big\Vert \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b})\Big\Vert^2\right]
    \\&\leq \left(\frac{E_i-1}{E_i}\right)^2 \Big\Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Big\Vert^2.
    \end{aligned}
\end{equation}
Replacing the above results in~\eqref{eq:66} yields:
\begin{equation}
    \begin{aligned}
    \mathbb{E}\Vert \epsilon \Vert^2 \leq& 2\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
    \end{aligned}
\end{equation}
Replacing the above result in~\eqref{eq:65}, we get:
  \begin{equation}\label{eq:65_1}
     \begin{aligned}
        \mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]-f_i(\mathbf{w}^{(k-1)}_{i,e-2})&\leq \mu\left({L\eta^2} -2\eta\right) \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
 Adding $f_i(\mathbf{w}^{(k-1)}_{i,e-2})$ to and subtracting $f_i(\mathbf{w}^{(k-1)^\star}_i)$ from both hand sides of the above inequality results in the following bound:
 \begin{equation}\label{eq:71}
     \begin{aligned}
        \mathbb{E}_{e-2} [f_i(\mathbf{w}^{(k-1)}_{i,e-1})]-f_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \left({L\mu\eta^2} -2\eta\mu+1\right) \left(f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k)}_{i,e-2}- \mathbf{w}^{(k)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
Since the local function is L-smooth, we get:
\begin{equation}
    f_i(\mathbf{w}^{(k-1)}_{i,e-2})- f_i(\mathbf{w}^{(k-1)^\star}_i) \leq \frac{L}{2} \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2,
\end{equation}
Also, since the local function is strong convex, we have:
\begin{equation}
\frac{\mu}{2}    \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2  \leq  f_i(\mathbf{w}^{(k-1)}_{i,e-1})- f_i(\mathbf{w}^{(k-1)^\star}_i).
\end{equation}
Replacing the above two results in~\eqref{eq:71} results in the following bound:
 \begin{equation}\label{eq:74}
     \begin{aligned}
        \frac{\mu}{2}    \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq& \left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \\ &+\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)\Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i\Vert^2\\&
     +{L}\eta^2\Bigg(\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\&+ \left(\frac{E_i-1}{E_i}\right)^2 \Vert \mathbf{w}^{(k-1)}_{i,e-2}-\mathbf{w}^{{(k-1)}^\star}_{i}\Vert^2\Bigg).
     \end{aligned}
 \end{equation}
Equivalently, we have:
 \begin{equation}\label{eq:75}
     \begin{aligned}
        &   \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq\\& \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2\left( \left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} +\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)+L\eta^2\left(\frac{E_i-1}{E_i}\right)^2\right)\frac{2}{\mu}  \\&
     +\frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}.
     \end{aligned}
 \end{equation}
We define the following two quantities to simplify the above expression:
 \begin{equation}
     \begin{aligned}
       \Psi_i \triangleq \left(\left({L\mu\eta^2} -2\eta\mu+1\right) \frac{L}{2} +\left(1-L\eta \right)\eta L^2 \left(\frac{E_i-1}{E_i}\right)+L\eta^2\left(\frac{E_i-1}{E_i}\right)^2\right)\frac{2}{\mu} ,
     \end{aligned}
 \end{equation}
  \begin{equation}\label{eq:77}
     \begin{aligned}
  \theta_i( \mathbf{w}^{(k-1)}_{i,e-2})\triangleq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)},
     \end{aligned}
 \end{equation}
 where $\Theta_i( \mathbf{w}^{(k-1)}_{i,e-2})$ corresponds to diversity of data at the node. More specifically, it measures the square error of gradient evaluated at individual local datapoints. It is evident that as the distribution of local data becomes more homogeneous this quantity decreases. 
 Using Assumption~\ref{Assump:DataVariabilit}, we get:
 \begin{equation}
 \begin{aligned}
    & \theta_i( \mathbf{w}^{(k-1)}_{i,e-2})= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right\Vert^2}{B_i(D_i-1)}\\
     &= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i} \left\Vert\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\frac{1}{D_i}\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &= \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{1}{D^2_i} \left\Vert D_i\nabla  f_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b}) -\sum_{b'\in\mathcal{D}_i}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2},x_{i,b'})\right\Vert^2}{B_i(D_i-1)}
     \\
     &\leq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{\sum_{b=1}^{D_i}\frac{(D_i-1)}{D_i} \Theta_i}{B_i(D_i-1)}=\frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}.
     \end{aligned}
 \end{equation}
 Let $\varrho_i \triangleq \frac{2}{\mu} {L}\eta^2\left(1-\frac{B_i}{D_i} \right) \frac{ \Theta_i}{B_i}$. By replacing the above results in~\eqref{eq:75}, we get:
 \begin{equation}\label{eq:80}
     \begin{aligned}
       \mathbb{E}_{e-2} \Vert \mathbf{w}^{(k-1)}_{i,e-1}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}_{i,e-2}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi_i  + \varrho_i.
     \end{aligned}
 \end{equation}
 The above expression is the one step decrease of the  local function during the period of local updates. Recursively expanding the above expression, since the local iterations starts with receiving the model parameter $\mathbf{w}^{(k-1)}$ from the server, i.e., $\mathbf{w}^{(k-1)}_{i,0}=\mathbf{w}^{(k-1)}$, we get:
  \begin{equation}
     \begin{aligned}
       \mathbb{E} \Vert \mathbf{w}^{(k-1)}_{i,e}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{e}_i  + \sum_{j=0}^{e-1}\Psi^{j}_i\varrho_i,
     \end{aligned}
 \end{equation}
which is equivalent to:
  \begin{equation}
     \begin{aligned}
       \mathbb{E} \Vert \mathbf{w}^{(k-1)}_{i,e}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{e}_i  + \varrho_i\frac{1-\Psi^{e}_i}{1-\Psi_i}, ~e\geq 1.
     \end{aligned}
 \end{equation}
As a result, we have:
 \begin{equation}
     \begin{aligned}
       \mathbb{E} \Vert \mathbf{w}^{(k-1)}_{i,E}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \leq \Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E}_i  + \varrho_i\frac{1-\Psi^{E}_i}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
 Considering the global weight update as follows:
 
\begin{equation}\label{eq:globAgg}
    \mathbf{w}^{(k)}=\frac{1}{N}\sum_{i=1}^{N} \mathbf{w}^{(k-1)}_{i,E_i},
\end{equation}
we have:
\begin{equation}\label{eq:globAgg}
\begin{aligned}
   \mathbb{E} &\left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2=\mathbb{E}\left\Vert \frac{1}{N}\sum_{i=1}^{N} \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2= \mathbb{E}\left\Vert \sum_{i=1}^{N}\frac{1}{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2=\frac{1}{N^2} \mathbb{E}\left\Vert \sum_{i=1}^{N} \left[\mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star}\right] \right\Vert^2
   \\&
   \overset{(i)}{\leq} \frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}- \mathbf{w}^{{(k)}^\star} \right\Vert^2=\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} + \mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star}+\mathbf{w}^{{(k-1)}^\star}-\mathbf{w}^{{(k)}^\star} \right\Vert^2
   \\
   & \overset{(ii)}{\leq}\frac{3}{N}\sum_{i=1}^{N}\left[\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} \right\Vert^2+\left\Vert\mathbf{w}_i^{{(k-1)}^\star} -\mathbf{w}^{{(k-1)}^\star} \right\Vert^2+ \left\Vert\mathbf{w}^{{(k-1)}^\star} -\mathbf{w}^{{(k)}^\star} \right\Vert^2\right]\\&= \frac{3}{N}\sum_{i=1}^{N}\mathbb{E}\left\Vert  \mathbf{w}^{(k-1)}_{i,E_i}-  \mathbf{w}_i^{{(k-1)}^\star} \right\Vert^2+\frac{3}{N}\sum_{i=1}^{N}\xi_i+3\Delta_m^2 \\
   \\
   & \overset{(ii)}{\leq} \frac{3}{N}\sum_{i=1}^{N}\left[\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E}_i  + \varrho_i\frac{1-\Psi^{E}_i}{1-\Psi_i}\right]+\frac{3}{N}\sum_{i=1}^{N}\xi_i+3\Delta_m^2 \\&=\frac{3}{N}\sum_{i=1}^{N}\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star}_i \Vert^2 \Psi^{E}_i +\frac{3}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E}_i}{1-\Psi_i}\right]+3\Delta_m^2
   \\&\overset{(iii)}{\leq} \frac{6}{N}\sum_{i=1}^{N}\left[\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2 \Psi^{E}_i  + \Vert \mathbf{w}^{(k-1)^\star} - \mathbf{w}^{(k-1)^\star}_i \Vert^2\Psi^{E}_i\right]+\frac{3}{N}\sum_{i=1}^{N}\left[ \xi_i+ \varrho_i\frac{1-\Psi^{E}_i}{1-\Psi_i}\right]+3\Delta_m^2\\&={6\Psi^{E}_i }\Vert \mathbf{w}^{(k-1)}- \mathbf{w}^{(k-1)^\star} \Vert^2  +\underbrace{\frac{3}{N}\sum_{i=1}^{N}\left[\xi_i(1+2\Psi^{E}_i)+ \varrho_i\frac{1-\Psi^{E}_i}{1-\Psi_i}\right]+3\Delta_m^2}_{\triangleq  \nu}.
   \end{aligned}
   \hspace{-7mm}
\end{equation}
where in (i),(ii),(iii) we used Cauchy–Schwarz inequality
Recursively expanding the above term gives us:
\begin{equation}
    \begin{aligned}
     \mathbb{E} \left\Vert\mathbf{w}^{(k)} - \mathbf{w}^{{(k)}^\star}\right\Vert^2&\leq {\left(6\Psi^{E}_i \right)^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \sum_{j=0}^{k-1}  \left(6\Psi^{E}_i \right)^{j}
     \\&={\left(6\Psi^{E}_i \right)^k}\Vert \mathbf{w}^{(0)}- \mathbf{w}^{(0)^\star} \Vert^2  + \nu \frac{1-\left(6\Psi^{E}_i\right)^k}{1-6\Psi^{E}_i}.\end{aligned}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 \end{proof}

==> proofThStrat.tex <==
\section{Proof of Theorem~\ref{th:straMain}}

For each local function, for $e\geq 2$ we can write the update as:
\begin{equation}
\begin{aligned}
    &\mathbf{w}^{(k-1)}_{i,e-1}=  \mathbf{w}^{(k-1)}_{i,e-2} - \frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{d\in \mathcal{B}^{(k),e}_{i,j}}  \frac{|\mathcal{S}^{(k)}_{i,j}|\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|}\\
    &= \mathbf{w}^{(k)}_{i,e-2} -  \frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)
    \\&+\underbrace{\left(\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d) -\frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}}\sum_{d\in \mathcal{B}^{(k),e}_{i,j}}  \frac{|\mathcal{S}^{(k)}_{i,j}|\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|} \right)}_{\triangleq \epsilon_i},
    \end{aligned}
\end{equation}
In the above format, the local updates are written in terms of conducting a full batch GD with an added noise that is due to the stratified-based minibatch SGD.
Since the local loss function is L-smooth, using the first order Taylor expansion, we get:
\begin{equation}\label{eq:quadBound}
 \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ (\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2})^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})+\frac{L}{2}\norm{\mathbf{w}^{(k-1)}_{i,e-1}-\mathbf{w}^{(k-1)}_{i,e-2}}^2.
     \end{aligned}
 \end{equation}
 Consequently, we have:
 \begin{equation}
      \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ (-\eta_i^{(k)}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i)^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\norm{-\eta_i^{(k)}\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2}) + \epsilon_i}^2.
     \end{aligned}
 \end{equation}
 Performing some algebraic manipulations on the above inequality yields:
  \begin{equation}
      \begin{aligned}
     F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})- \eta_i^{(k)} \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \epsilon_i^\top \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\\&
     +\frac{L}{2}\left(\left(\eta_i^{(k)}\right)^2\Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2+\Vert \epsilon_i\Vert^2-2\eta_i^{(k)} \epsilon_i^\top\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\right).
     \end{aligned}
 \end{equation}
 Thus, we get:
 \begin{equation}\label{eq:59}
     \begin{aligned}
         F_i(\mathbf{w}^{(k-1)}_{i,e-1})\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\left(\eta_i^{(k)}\right)^2}{2} -\eta_i^{(k)}\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 + \left(1-L\eta_i^{(k)} \right)\epsilon_i^{\top} \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\Vert \epsilon_i\Vert^2.
     \end{aligned}
 \end{equation}
 Taking the expectation from both hand sides of the above inequality, we have:
  \begin{equation}\label{eq:106}
     \begin{aligned}
        \mathbb{E}_{e-2} [ F_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\left(\eta_i^{(k)}\right)^2}{2} -\eta_i^{(k)}\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 \\
        &+ \left(1-L\eta_i^{(k)} \right)\underbrace{\mathbb{E}_{e-2} [\epsilon_i^{\top}]}_{\eqref{eq:106}-(a)} \nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})
     +\frac{L}{2}\underbrace{\mathbb{E}_{e-2} [\Vert \epsilon_i\Vert^2]}_{\eqref{eq:106}-(b)}.
     \end{aligned}
 \end{equation}
 To calculate $\eqref{eq:106}-(a)$, we take the following steps:
 \begin{equation}\label{eq:107}
 \begin{aligned}
     \mathbb{E}_{e-2} [\epsilon_i]&=\mathbb{E}_{e-2} \left[\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d) -\frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}}\sum_{d\in \mathcal{B}^{(k),e}_{i,j}}  \frac{|\mathcal{S}^{(k)}_{i,j}|\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|}\right]\\
     &=\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)-\mathbb{E}_{e-2}\left[ \frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}}\sum_{d\in \mathcal{B}^{(k),e}_{i,j}}  \frac{|\mathcal{S}^{(k)}_{i,j}|\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|}\right]
     \\&=\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)- \frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}}|\mathcal{S}^{(k)}_{i,j}| \mathbb{E}_{e-2}\left[\sum_{d\in \mathcal{B}^{(k),e}_{i,j}} \frac{\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|}\right]\\&
     \overset{\eqref{eq:107}-(a)}=\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)- \frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \sum_{d\in \mathcal{S}^{(k)}_{i,j}}\frac{\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{S}^{(k)}_{i,j}|}
     \\&=\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)- \frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \sum_{d\in \mathcal{S}^{(k)}_{i,j}}{\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}=0
     \end{aligned}
 \end{equation}
 where $\eqref{eq:107}-(a)$ is due to the fact that inside each strata, we perform uniform sampling without replacement.
 
Now, we aim to calculate $\eqref{eq:106}-(b)$. We first consider the result of~\cite{lohr2019sampling} (Chapter 3, Eq. (3.5)), using a similar approach the following relationship can be obtained:
\begin{equation}\label{eq:108}
 \begin{aligned}
     \mathbb{E}_{e-2} [\Vert\epsilon_i\Vert^2]&=\mathbb{E}_{e-2} \left[\left\Vert\frac{\eta_i^{(k)}}{D^{(k)}_i} \sum_{d\in\mathcal{D}^{(k)}_i} \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d) -\frac{\eta_i^{(k)}}{|\mathcal{D}^{(k)}_i|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}}\sum_{d\in \mathcal{B}^{(k),e}_{i,j}}  \frac{|\mathcal{S}^{(k)}_{i,j}|\nabla  f_i(\textbf{w}^{(k),e-1}_{i},d)}{|\mathcal{B}^{(k),e}_{i,j}|}\right\Vert^2\right]\\
     &=\left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(1-\frac{|\mathcal{B}^{(k)}_{i,j}|}{|\mathcal{S}^{(k)}_{i,j}|} \right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|}.
     \end{aligned}
 \end{equation}
 which hold regardless of the choice of the minibatch selections, i.e., $\mathcal{B}^{(k)}_{i,j}$, $\forall i,j$. We now apply the condition in~\eqref{eq:allocMini}, which gives us:
 \begin{equation}\label{eq:109}
 \begin{aligned}
     \mathbb{E}_{e-2} [\Vert\epsilon_i\Vert^2]&=\left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{1}{|\mathcal{B}^{(k)}_{i,j}|}-\frac{1}{|\mathcal{S}^{(k)}_{i,j}|} \right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}\\&=\left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{1}{|\mathcal{B}^{(k)}_{i,j}|}-\frac{1}{|\mathcal{S}^{(k)}_{i,j}|} \right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}\\
     &=\left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{\sum_{\mathcal{S}^{(k)}_{i,j'}\in \mathcal{S}^{(k)}_{i}} \sigma(\mathcal{S}^{(k)}_{i,j'})\vert \mathcal{S}^{(k)}_{i,j'}\vert }{ |\mathcal{B}^{(k),e}_{i}|\sigma(\mathcal{S}^{(k)}_{i,j})\vert \mathcal{S}^{(k)}_{i,j}\vert }\right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}-\left(\frac{1}{|\mathcal{S}^{(k)}_{i,j}|} \right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}\\&
     \leq \left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{\sum_{\mathcal{S}^{(k)}_{i,j'}\in \mathcal{S}^{(k)}_{i}} \sigma(\mathcal{S}^{(k)}_{i,j'})\vert \mathcal{S}^{(k)}_{i,j'}\vert }{ |\mathcal{B}^{(k),e}_{i}|\sigma(\mathcal{S}^{(k)}_{i,j})\vert \mathcal{S}^{(k)}_{i,j}\vert }\right)|\mathcal{S}^{(k)}_{i,j}|^2 \frac{\sigma^2(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}\\&
     =\left(\eta_i^{(k)}\right)^2  \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{\sum_{\mathcal{S}^{(k)}_{i,j'}\in \mathcal{S}^{(k)}_{i}} \sigma(\mathcal{S}^{(k)}_{i,j'})\vert \mathcal{S}^{(k)}_{i,j'}\vert }{ |\mathcal{B}^{(k),e}_{i}| }\right)|\mathcal{S}^{(k)}_{i,j}| \frac{\sigma(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}\\&
     =\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\sum_{\mathcal{S}^{(k)}_{i,j'}\in \mathcal{S}^{(k)}_{i}} \sigma(\mathcal{S}^{(k)}_{i,j'})\vert \mathcal{S}^{(k)}_{i,j'}\vert \right)|\mathcal{S}^{(k)}_{i,j}| \frac{\sigma(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|^2}
     \\&=\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} \left(\frac{\sum_{\mathcal{S}^{(k)}_{i,j'}\in \mathcal{S}^{(k)}_{i}} \sigma(\mathcal{S}^{(k)}_{i,j'})\vert \mathcal{S}^{(k)}_{i,j'}\vert}{{|\mathcal{B}^{(k)}_{i,j}|}} \right)|\mathcal{S}^{(k)}_{i,j}| \frac{\sigma(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|}=\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \left(\sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \frac{\sigma(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|} \right)^2.
     \end{aligned}
     \hspace{-7mm}
 \end{equation}
 Now, note that we can bound the as follows:
 \begin{equation}\label{eq:110}
 \begin{aligned}
     \sigma(\mathcal{S}^{(k)}_{i,j})&= \sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} } \Big\Vert \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)-{\sum_{d'\in\mathcal{S}^{(k)}_{i,j}} }\frac{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d')}{|\mathcal{S}^{(k)}_{i,j}|}\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}} \\
     &=\sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} }\frac{1}{|\mathcal{S}^{(k)}_{i,j}|^2} \Big\Vert |\mathcal{S}^{(k)}_{i,j}|\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)-{\sum_{d'\in\mathcal{S}^{(k)}_{i,j}} }{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d')}\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}\\
     &\overset{\eqref{eq:110}-(a)}{\leq} \sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} }\frac{|\mathcal{S}^{(k)}_{i,j}|-1}{|\mathcal{S}^{(k)}_{i,j}|^2} \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \Big\Vert \nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d)-{ }{\nabla f_i(\mathbf{w}^{(k-1)}_{i,e-2},d')}\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}
     \\&\leq \sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} }\frac{(|\mathcal{S}^{(k)}_{i,j}|-1)\widetilde{L}^2}{|\mathcal{S}^{(k)}_{i,j}|^2} \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \Big\Vert d-d'\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}\leq \sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} }\frac{\widetilde{L}^2}{|\mathcal{S}^{(k)}_{i,j}|} \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \Big\Vert d-d'\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}
     \\& \leq \frac{\widetilde{L}}{\sqrt{|\mathcal{S}^{(k)}_{i,j}|}}\sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} } \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \Big\Vert d-d'\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}\\
     &\overset{\eqref{eq:110}-(b)}{\leq}\frac{\widetilde{L}}{\sqrt{|\mathcal{S}^{(k)}_{i,j}|}}\sqrt{\frac{2\sum_{d\in\mathcal{S}^{(k)}_{i,j} } \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \left[\Big\Vert d-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|} \Big\Vert^2 + \Big\Vert d'-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|}\Big\Vert^2 \right]}{|\mathcal{S}^{(k)}_{i,j}|-1}}
     \\&=\frac{\sqrt{2}\widetilde{L}}{\sqrt{|\mathcal{S}^{(k)}_{i,j}|}}\sqrt{\frac{\sum_{d\in\mathcal{S}^{(k)}_{i,j} } \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \left[\Big\Vert d-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|} \Big\Vert^2 + \Big\Vert d'-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|}\Big\Vert^2 \right]}{|\mathcal{S}^{(k)}_{i,j}|-1}}
     \\&=\frac{\sqrt{2}\widetilde{L}}{\sqrt{|\mathcal{S}^{(k)}_{i,j}|}}\sqrt{\frac{ |\mathcal{S}^{(k)}_{i,j}| \sum_{d\in\mathcal{S}^{(k)}_{i,j} } \Big\Vert d-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|} \Big\Vert^2 +  |\mathcal{S}^{(k)}_{i,j}| \sum_{d'\in\mathcal{S}^{(k)}_{i,j}} \Big\Vert d'-  \frac{\sum_{d''\in\mathcal{S}^{(k)}_{i,j}}d''}{|\mathcal{S}^{(k)}_{i,j}|}\Big\Vert^2}{|\mathcal{S}^{(k)}_{i,j}|-1}}
     \\&=\frac{\sqrt{2}\widetilde{L}}{\sqrt{|\mathcal{S}^{(k)}_{i,j}|}}\sqrt{2
     |\mathcal{S}^{(k)}_{i,j}| }
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})={{2}\widetilde{L}}
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})
     \end{aligned}
 \end{equation}
 where in $\eqref{eq:110}-(a),(b)$, we have used the Cauchy-Schwarz inequality.
 
 
Replacing the above inequality in~\eqref{eq:109}, gives us:
\begin{equation}\label{eq:111}
    \mathbb{E}_{e-2} [\Vert\epsilon_i\Vert^2]\leq \frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \left(\sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \frac{{{2}\widetilde{L}}
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|} \right)^2
\end{equation}
Replacing~\eqref{eq:111},\eqref{eq:107} in \eqref{eq:106}, we get:
\begin{equation}\label{eq:112}
     \begin{aligned}
        \mathbb{E}_{e-2} [ F_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq& F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \left(\frac{L\left(\eta_i^{(k)}\right)^2}{2} -\eta_i^{(k)}\right) \Vert\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})\Vert^2 \\
        &
     +2L\widetilde{L}\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \left(\sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \frac{
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|} \right)^2.
     \end{aligned}
 \end{equation}
  To avoid sign change in the second term of the right hand side, we 
 tune the step size such that $\frac{L\left(\eta_i^{(k)}\right)^2}{2} -\eta_i^{(k)} <0$, implying $\eta_i^{(k)} \leq 2/L$. Using the PL condition, we have:
 \begin{equation}
        \norm{\nabla F_i(\mathbf{w}^{(k-1)}_{i,e-2})}^2 \geq \left(F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right){2\mu},
 \end{equation}
 where $\mathbf{w}^{(k-1)^\star}_i$ denotes the local optimal point of the local dataset at node $i$.
 Replacing the above result in~\eqref{eq:62}, we get:
  \begin{equation}\label{eq:65}
     \begin{aligned}
        &\mathbb{E}_{e-2} [F_i(\mathbf{w}^{(k-1)}_{i,e-1})]\leq F_i(\mathbf{w}^{(k-1)}_{i,e-2})+ \mu\left({L\left(\eta_i^{(k)}\right)^2} -2\eta_i^{(k)}\right)  (F_i(\mathbf{w}^{(k-1)}_{i,e-2})- F_i(\mathbf{w}^{(k-1)^\star}_i)) 
     \\&+2L\widetilde{L}\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \left(\sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \frac{
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|} \right)^2.
     \end{aligned}
 \end{equation}
 Adding $F_i(\mathbf{w}^{(k-1)}_{i,e-2})$ and subtracting $F_i(\mathbf{w}^{(k-1)^\star}_i)$ from both hand sides and recursively expanding the resulting expression up to the time of previous global aggregation, we get:
 \begin{equation}
     \begin{aligned}
        \mathbb{E} [F_i(\mathbf{w}^{(k-1)}_{i,E})]-F_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \left(\underbrace{{L\mu\left(\eta_i^{(k)}\right)^2} -2\eta_i^{(k)}\mu+1}_{\triangleq \Psi_i}\right)^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right) \\&
     +\underbrace{2L\widetilde{L}\frac{\left(\eta_i^{(k)}\right)^2 }{ |\mathcal{B}^{(k),e}_{i}|} \left(\sum_{\mathcal{S}^{(k)}_{i,j}\in \mathcal{S}^{(k)}_{i}} |\mathcal{S}^{(k)}_{i,j}| \frac{
     \widetilde{\sigma}(\mathcal{S}^{(k)}_{i,j})}{|\mathcal{B}^{(k)}_{i,j}|} \right)^2}_{\triangleq \varrho_i} \sum_{j=0}^{E-1}\left({L\mu\left(\eta_i^{(k)}\right)^2} -2\eta_i^{(k)}\mu+1\right)^j,
     \end{aligned}
 \end{equation}
 which is equivalent to:
 \begin{equation}
     \begin{aligned}
        \mathbb{E} [F_i(\mathbf{w}^{(k-1)}_{i,E})]-F_i(\mathbf{w}^{(k-1)^\star}_i)\leq& \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}.
     \end{aligned}
 \end{equation}
 Consider the global function as follows (for simplicity the number of data points are assumed to be the same for now!):
 \begin{equation}
    F(\mathbf{w}^{(k)})= \frac{1}{N} \sum_{i \in \mathcal{N}}  F_{n}(\textbf{w}^{(k)}),
\end{equation}
we have:
 \begin{equation}
 \hspace{-7mm}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})&= \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F(\mathbf{w}^{{(k)}^\star}) \right]\\&= \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F_i(\mathbf{w}^{{(k-1)}^\star}_{i})+F_i(\mathbf{w}^{{(k-1)}^\star}_{i})-F_i(\mathbf{w}^{{(k)}^\star}_{i})+F_i(\mathbf{w}^{{(k)}^\star}_{i})-F(\mathbf{w}^{{(k)}^\star}) \right]\\&
    \leq\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ F_i(\mathbf{w}^{(k-1)}_{i,E})-F_i(\mathbf{w}^{{(k-1)}^\star}_{i})+\Delta_i+\xi_i \right]\\&
    \leq\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i \right]\\&
    =\frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})- F_i(\mathbf{w}^{(k-1)^\star}_i)+F_i(\mathbf{w}^{(k-1)^\star})-F_i(\mathbf{w}^{(k-1)^\star})\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i \right]\\&=
     \frac{1}{N} \sum_{i \in \mathcal{N}} \left[ \Psi_i^{E_i} \left(F_i(\mathbf{w}^{(k-1)})-F_i(\mathbf{w}^{(k-1)^\star})\right)
     +\varrho_i\frac{1-\Psi_i^{E_i}}{1-\Psi_i}+\Delta_i+\xi_i(1-\Psi_i^{E_i}) \right].
    \end{aligned}
    \hspace{-7mm}
\end{equation}
 Assuming the same step size among the nodes, i.e., $\Psi_i=\Psi\triangleq (1-2\eta\mu+L\eta^2\mu)$, $\forall i$, and the same epoch sizes, i.e., $E_i=E$, we have:
  \begin{equation}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})\leq
    \Psi^{E}\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right)
     +\underbrace{\frac{1}{N} \sum_{i \in \mathcal{N}} \left[\varrho_i\frac{1-\Psi^{E}}{1-\Psi}+\Delta_i+\xi_i(1-\Psi^{E})\right]}_{\triangleq \nu}.
    \end{aligned}
\end{equation}
Recursively expanding the above expression yields:
\begin{equation}
     F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})\leq
    \Psi^{E\times k}\left(F(\mathbf{w}^{(0})- F(\mathbf{w}^{(0)^\star})\right)
     +\nu \frac{1-\Psi^{E\times k}}{1-\Psi^{E}}.
\end{equation}


---- Successive term cancellation:
Consider the relationship:
 \begin{equation}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})\leq
    \Psi^{E}\left(F(\mathbf{w}^{(k-1)})- F(\mathbf{w}^{(k-1)^\star})\right)
     +\nu.
    \end{aligned}
\end{equation}
This can be expanded as:
 \begin{equation}
 \begin{aligned}
    F(\mathbf{w}^{(k)})-F(\mathbf{w}^{{(k)}^\star})&\leq
    \Psi^{E}\left(\Psi^{E}\left(F(\mathbf{w}^{(k-2)})- F(\mathbf{w}^{(k-2)^\star})+\nu\right)\right)
     +\nu
     \\&=\Psi^{2E}\left(F(\mathbf{w}^{(k-2)})- F(\mathbf{w}^{(k-2)^\star})\right)
     +\nu(
    \end{aligned}
\end{equation}
